Penetrating Shields: A Systematic Analysis of Memory Corruption Mitigations in the Spectre Era

This paper provides the first systematic analysis of a synergistic threat model encompassing memory corruption vulnerabilities and microarchitectural side-channel vulnerabilities. We study speculative shield bypass attacks that leverage speculative execution attacks to leak secrets that are critical to the security of memory corruption mitigations (i.e., the shields), and then use the leaked secrets to bypass the mitigation mechanisms and successfully conduct memory corruption exploits, such as control-flow hijacking. We start by systematizing a taxonomy of the state-of-the-art memory corruption mitigations focusing on hardware-software co-design solutions. The taxonomy helps us to identify 10 likely vulnerable defense schemes out of 20 schemes that we analyze. Next, we develop a graph-based model to analyze the 10 likely vulnerable defenses and reason about possible countermeasures. Finally, we present three proof-of-concept attacks targeting an already-deployed mitigation mechanism and two state-of-the-art academic proposals.

==> sections/analysis-old.tex <==




%\begin{figure*}[t]
%    \centering
%    \includegraphics[width=\textwidth]{figures/flowchart.pdf}
%    \caption{Taxonomy of memory corruption mitigations.}
%    \label{fig:flowchart}
%\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{comment}
\begin{table*}[]
\footnotesize
\begin{center}
\begin{tabular}{|l|clll
>{\columncolor[HTML]{FFCB2F}}c |}
\hline
 &
  \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Memory Corruption Mitigations}} \\ \cline{2-6} 
 &
  \multicolumn{4}{c|}{\textbf{Address Augmentation}} &
  \cellcolor[HTML]{FFCC67} \\ \cline{2-5}
\multirow{-3}{*}{Category} &
  \multicolumn{2}{c|}{\textbf{Tamperproof Metadata}} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{FFCC67}\textbf{Tamperable Metadata}} &
  \multirow{-2}{*}{\cellcolor[HTML]{FFCC67}\begin{tabular}[c]{@{}c@{}}\textbf{Address Layout} \\ \textbf{Randomization}\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Mitigation \\ Examples\end{tabular} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Full Information:\\ 
  - CHERI~\cite{cheri}\\ 
  - Intel MPX~\cite{intelmpx}\\ 
  - HardBound~\cite{hardbound}\\ 
  - Watchdog~\cite{watchdog}\\ 
  - WatchdogLite~\cite{watchdoglite}\\ 
  - CHEx86~\cite{chex86}\\ 
  - No-FAT~\cite{no-fat}$\ddagger$
  \end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Partial Information:\\ 
  - Intel CET~\cite{intelcet}\\ 
  - ARM BTI~\cite{armbti}\\ 
  - ZERO~\cite{zero}\\ 
  - REST~\cite{rest}\\ 
  - Califorms~\cite{califorms}$\dagger$
  \end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}\begin{tabular}[c]{@{}l@{}}Function of Pointer:\\ 
  - ARM PA~\cite{armpa}\\ 
  - AOS~\cite{aos}\\ 
  - C3~\cite{c3}
  \end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}\begin{tabular}[c]{@{}l@{}}Random Number:\\ 
  - ARM MTE~\cite{armmte}\\ 
  - SPARC ADI~\cite{sparc_adi}\\ 
  - No-FAT~\cite{no-fat}$\ddagger$ \\ 
  - Stack Smashing \\    
  Protection~\cite{stackguard_canaries}
  \end{tabular}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFCC67}\begin{tabular}[c]{@{}l@{}}
  - ASLR~\cite{pax_aslr, usenix_aslr}\\ 
  - Morpheus~\cite{morpheus}\\ 
  - Califorms~\cite{califorms}$\dagger$
  \end{tabular}} \\ \hline
\end{tabular}
\end{center}
\vspace{-5pt}
{\small \textsuperscript{$\dagger$}Califorms maintains tamperproof metadata for adjacent vulnerability protection and adds randomness to the size of the metadata
%\mengjia{completely depends on how to define metadata... do you call the redzone content metadata?}\weon{i meant the size of the security bytes. The content is not metadata. More like the location} 
for non-adjacent vulnerability protection; the randomness regarding the size of the metadata is vulnerable to information disclosure attacks.
\textsuperscript{$\ddagger$}No-FAT maintains tamperproof metadata for spatial protection, but tamperable metadata for temporal protection; the tamperable metadata is vulnerable to information disclosure attacks.
}
\caption{
Taxonomy of memory corruption mitigations. The highlighted mechanisms are vulnerable to information disclosure attacks.
%\mengjia{is it possible to make these texts smaller?}
%\weon{moved them to footnote. not sure if this is better tho.}
}
\mengjia{change this table. I am thinking that we do not need to distinguish between full information and partial information, no need to distinguish between function poiter and random nubmer..}

\label{tab:taxonomy}
%\mengjia{1. let's add star/dagger to ``No-FAT'' and ``Califorms'' and put footnote of this table.\\
%2. add a column to the left, for the first three rows -> put category, and for the last row -> put mitigation examples. You can rotate the text if possible.}
\end{table*}
\end{comment}

\begin{comment}
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
every node/.style = {draw=black, 
	inner color=gray!5,
	outer color=gray!10,
	fill = yellow,
	rounded corners, 
	thick,
	text width=49mm, 
	minimum width=1cm,
	%rounded corners=3,
	%text height=1.5ex,
	%text depth=0ex,
	align=center,
	anchor=north, 
	font=\footnotesize},
level distance = 6mm,
sibling distance = 82mm,
edge from parent fork down
]
\node {Memory Corruption Mitigations}
child{ node {Address Augmentation}[sibling distance = 54mm]
    child{ node {Tamperproof Metadata Augmentation}
    	child{ node {CHERI~\cite{cheri}, Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog},
    	WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86},
    	Intel CET~\cite{intelcet}, ARM BTI~\cite{armbti}, ZERO~\cite{zero}, REST~\cite{rest},
    	Califorms$\dagger$~\cite{califorms}, No-FAT$\ddagger$~\cite{no-fat} }}
    }
    child{ node {{\textcolor{red}{Tamperable Metadata Augmentation}}}
    	child{ node {
    	{\textcolor{red}{Stack Smashing Protection}}~\cite{stackguard_canaries}, 
    	{\textcolor{red}{ARM PA}}~\cite{qualcomm_white_paper}, 
    	{\textcolor{red}{ARM MTE}}~\cite{armmte}, 
    	{\textcolor{red}{AOS}}~\cite{aos}, 
    	{\textcolor{red}{C3}}~\cite{c3}, {\textcolor{red}{No-FAT$\ddagger$}}~\cite{no-fat}}}
    }
}
child{ node {{\textcolor{red}{Address Layout Randomization}}}
	child{ node {
	{\textcolor{red}{ASLR}}~\cite{pax_aslr, usenix_aslr}, {\textcolor{red}{Califorms$\dagger$}}~\cite{califorms}, {\textcolor{red}{Morpheus}}~\cite{morpheus} }}
};
\end{tikzpicture}
{\newline\footnotesize \textsuperscript{$\dagger$}Califorms maintains tamperproof metadata for adjacent vulnerability protection and adds randomness to the size of the metadata
%\mengjia{completely depends on how to define metadata... do you call the redzone content metadata?}\weon{i meant the size of the security bytes. The content is not metadata. More like the location} 
for non-adjacent vulnerability protection; the randomness regarding the size of the metadata is vulnerable to \ssb attacks.
\newline\textsuperscript{$\ddagger$}No-FAT maintains tamperproof metadata for spatial protection, but tamperable metadata for temporal protection; the tamperable metadata is vulnerable to \ssb attacks.
}
	\caption{Taxonomy of proposed or deployed memory corruption mitigations when focusing on \ssb attacks. Mitigations in {\textcolor{red}{red}} are vulnerable to \ssb attacks.}
	\label{fig:taxonomy}
\end{figure*}
\end{comment}

\begin{figure*}[t]
\centering
\begin{tikzpicture}[
every node/.style = {draw=black, 
	inner color=gray!5,
	outer color=gray!10,
	fill = yellow,
	rounded corners, 
	thick,
	text width=49mm, 
	minimum width=1cm,
	%rounded corners=3,
	%text height=1.5ex,
	%text depth=0ex,
	align=center,
	anchor=north, 
	font=\footnotesize},
level distance = 6mm,
sibling distance = 82mm,
edge from parent fork down
]
\node {Memory Corruption Mitigations}
child{ node {\textcolor{red}{Spoofable Security Checks}}[sibling distance = 54mm]
    child{ node {{\textcolor{red}{Address Layout Randomization}}}
    	child{ node {
    	{\textcolor{red}{ASLR}}~\cite{pax_aslr, usenix_aslr}, {\textcolor{red}{Califorms$\dagger$}}~\cite{califorms}, {\textcolor{red}{Morpheus}}~\cite{morpheus} }}
    }
    child{ node {{\textcolor{red}{Tamperable Metadata Augmentation}}}
    	child{ node {
    	{\textcolor{red}{Stack Smashing Protection}}~\cite{stackguard_canaries}, 
    	{\textcolor{red}{ARM PA}}~\cite{qualcomm_white_paper}, 
    	{\textcolor{red}{ARM MTE}}~\cite{armmte}, 
    	{\textcolor{red}{AOS}}~\cite{aos}, 
    	{\textcolor{red}{C3}}~\cite{c3}, {\textcolor{red}{No-FAT$\ddagger$}}~\cite{no-fat} }}
    }
}
child{ node {Unspoofable Security Checks}
child{ node {Tamperproof Metadata Augmentation}
    child{ node {
	CHERI~\cite{cheri}, Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog},
	WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86},    	Intel CET~\cite{intelcet}, ARM BTI~\cite{armbti}, ZERO~\cite{zero}, REST~\cite{rest},
    Califorms$\dagger$~\cite{califorms}, No-FAT$\ddagger$~\cite{no-fat} }}
}
}
;
\end{tikzpicture}
{\newline\footnotesize \textsuperscript{$\dagger$}Califorms maintains tamperproof metadata for adjacent vulnerability protection and adds randomness to the size of the metadata
%\mengjia{completely depends on how to define metadata... do you call the redzone content metadata?}\weon{i meant the size of the security bytes. The content is not metadata. More like the location} 
for non-adjacent vulnerability protection; the randomness regarding the size of the metadata is vulnerable to \ssb attacks.
\newline\textsuperscript{$\ddagger$}No-FAT maintains tamperproof metadata for spatial protection, but tamperable metadata for temporal protection; the tamperable metadata is vulnerable to \ssb attacks.
}
	\caption{Taxonomy of proposed or deployed memory corruption mitigations when focusing on \ssb attacks. Mitigations in {\textcolor{red}{red}} are vulnerable to \ssb attacks.}
	\mengjia{move the comments to footnote? otherwise taking too much space?}
	\label{fig:taxonomy}
\end{figure*}


%\section{Systematic Analysis of Memory Corruption Mitigations against Synergistic Attacks}
\section{Systematic Security Analysis}
\label{sec:taxonomy}

\mengjia{maybe we need to change the section title.}

\begin{comment}
%\mengjia{I will try to draft the intro so the discussion will be easier here. 
%I would like to see whether we can organize these section by claiming our analysis is trying to answer a few questions:
%1) whether a mitigation mechanism is vulnerable to synergistic attacks;
%2) if so, what attack strategies can be used to break it; and how practical the attack will be}

The attack surface on modern systems extends across the system stack including vulnerabilities in both software (e.g., buffer overflows) and hardware (e.g., side channels). 
Due to the complexity of such a large attack surface, today's security researchers often delegate a large portion of the real attack surface as ``out of scope'' when devising a threat model for a particular defense proposal. 
Such a strategy ignores important synergies between the different threat models, overestimating the effectiveness of proposed mitigations. 

%\mengjia{after the new S3, I found this paragraph is a bit out of date...}
%\weon{should we remove it? Or fix it?}
%\mengjia{I removed a paragraph which used to be here... Need to check where we can include it back}
%\weon{Still flows well without it. I think we can remove it for good.}

%In this paper, we study the majority of new \mengjia{new? majority? I think we select those with some architectural components, we analyzed a few but did not analyze many software-only solutions} memory corruption mitigations that have been proposed in the academia~\cite{hardbound, watchdog, watchdoglite, aos, chex86, califorms, rest, morpheus, cheri, no-fat,zero,c3} and the industry~\cite{intelmpx, armmte,intelcet,armbti, armpa}, in the last decade. 

\mengjia{rewrite this paragraph.
1. mention there exist a lot of taxonomy/sok work, but none of them have focused on this specific angle.
2. set the scope of this section, the goal is not to have a comprehensive taxonomy.
a) look at software-hardware co-deisng; b) specifically look at how they can be bypassed via information leakage attacks, because side channel is an information leakage attack.
Put this reasoning in front, so people know the scope.}



\mengjia{I am thinking about what should come out of this section.
Instead of focusing on the metadata stuff, maybe we can try to formulate the security check in a general way, and then hint on the trustworthiness of the security check or authorization.
=> }

\begin{footnotesize}
\begin{verbatim}
- multiple works have analyzed/taxonomized memory corruption 
mitigations from a memory corruption attack angle.
- our goal is study from SSB angle.
- identify common weaknessses against SSBs.
- tamperproof
  - OOB shadow memory + OOB check for every memory access
  - tagged memory
  - page attributes
- tamperable
- address layout randomization.

\end{verbatim}
\end{footnotesize}
\end{comment}

%Despite the growing number of case studies demonstrating successful \ssb attacks~\cite{speculativeprobing, pacman}, there currently lacks a comprehensive study of memory corruption defenses against such attacks. 
%Past works~\cite{szekeres2013sok, novkovic2021} have developed taxonomies that allow one to better reason about the security of memory corruption defenses, but the taxonomies narrowly focus on memory corruption attacks and fail to shed light on their security against \ssb attacks. 
%As such, in this section, we aim to develop such a taxonomy; a taxonomy which allows one reason about the security of memory corruption mitigations against \ssb attacks. 
In this section, we aim to develop a taxonomy which allows one to reason about the security of memory corruption mitigations against \ssb attacks. 
Our ultimate goal is to identify and analyze a meaningful subset of the common weaknesses in memory corruption mitigations that may be exploited due to the presence of side-channel vulnerabilities in modern processors.

We start by first assessing the fundamental roots of current taxonomies of memory corruption defenses and why they are insufficient in analyzing these defenses against \ssb attacks.
Fundamentally, memory corruption vulnerabilities occur due to the lack of sufficient security checks in the vulnerable programs. 
Memory corruption defenses aim to protect these possibly vulnerable programs by augmenting them with automated security checks during their runtime. 
%As such, past taxonomies have tended to first develop comprehensive models of memory corruption attacks, and then categorize the defenses inside these attack models in relation to which steps of the attack the augmented security checks occur. 
As such, past taxonomies have tended to categorize the defenses inside memory corruption attack models, in relation to which steps of the attack the augmented security checks occur. 
While this approach is helpful in understanding which types of memory corruption attacks can be mitigated by the varying security checks imposed by the respective defenses, it is not as useful for understanding the resiliency of the defenses against \ssb attacks.

Recall from \cref{sec:threatmodel}, \ssb attacks 1) first perform an \emph{information disclosure} attack using a side-channel vulnerability to gain some secret knowledge and 2) then uses the leaked secret knowledge to \emph{spoof} the security check of a defense using a memory corruption vulnerability. In other words, from a \ssb attack perspective, it is not a question of which step of a memory corruption attack that a security check occurs in. Rather, the question is whether an attacker can attempt to forge rogue information that can spoof a security check, since this ultimately determines whether there is any incentive for an attacker to perform an information disclosure attack at all. 

We show our taxonomy in \cref{fig:taxonomy}  with examples of state-of-the-art mitigation mechanisms (focusing on hardware-software co-designs) from both academia\hbox{~\cite{hardbound, watchdog, watchdoglite, aos, chex86, califorms, rest, morpheus, cheri, no-fat,zero,c3, usenix_aslr}} and industry\hbox{~\cite{intelmpx, armmte,intelcet,armbti, armpa, pax_aslr}} for each category.
Mitigations in \textcolor{red}{red} are vulnerable to \ssb attacks.
We first divide mitigations depending on whether they perform \emph{spoofable} security checks (i.e., in the presence of an exploitable memory-write vulnerability, an attacker can forge rogue input to the security checks ) or \emph{unspoofable} security checks (i.e., the input to the security check cannot be controlled by an attacker). 

For spoofable security check based defenses, we further subdivide them depending on what kind of information is added for the additional security checks (i.e., what kind of information the attacker aims to leak). \emph{Address layout randomization} based defenses add random ``\emph{offsets}'' to the address of various (sub-)objects, entangling these offsets with the originally predictable (sub-)object addresses. On the other hand, \emph{tamperable metadata augmentation} based defenses augment addresses or pointers with additional information called ``\emph{metadata}'' that is maintained separately from the pointers. Since these defenses are spoofable for an attacker who is equipped with the correct offset or metadata, these defenses maintain this offset or metadata 1) as a \emph{secret} private to its security domain and 2) with high entropy. 

For unspoofable security check based defenses, we found that all defenses in this category can also be categorized as \emph{tamperproof metadata augmentation} based defenses which similarly augment addresses or pointers with additional information called ``\emph{metadata}''. However, they differ greatly in that they maintain unspoofable security checks by enforcing the integrity of their metadata. In fact, as the security checks are unspoofable, these defenses do not share the incentive of maintaining the privacy or high entropy of their metadata. Thus, the metadata in these defenses are generally public information (i.e., not secret), nullifying any merits of information disclosure. We now explain each category in more detail.

\paragraph{Address layout randomization} 
Address layout randomization based defenses randomize the position of (sub-)objects in virtual memory. 
To randomize the aforementioned addresses, these defenses add random offsets to the address of various (sub-)objects, entangling the offset with the originally predictable addresses.
The insight behind this approach is that if the addresses of (sub-)objects in the virtual memory are unknown, an adversary is unable to divert the control flow reliably, and thus can be caught using an illegal address (i.e., wrong offset) during a security check. When in action, security checks are performed for each memory access by first taking the memory address being accessed and checking whether the address is legal (i.e., the added offset is correct). 

Because a memory corruption exploit which overwrites a pointer allows an attacker to control the address (and hence the offset) being used for the security check, address layout randomization schemes can be categorized as performing spoofable security checks. To mitigate possible spoofing attempts from an attacker, address layout randomization schemes maintain the offset as a secret that is private to their security domain and with high entropy to mitigate guessing attempts. However, if side-channel vulnerabilities can be exploited to leak the secret offset from a victim's security domain to an attacker, then the attacker can next perform a memory corruption attack while leveraging this secret offset to successfully bypass address layout randomization defenses. Examples of address layout randomization schemes include ASLR~\cite{pax_aslr, usenix_aslr}, Morpheus~\cite{morpheus} and Califorms~\cite{califorms}. 


\paragraph{Tamperable Metadata Augmentation} 
Tamperable metadata augmentation based defenses augment addresses or pointers with separately maintained metadata. These metadata are used to perform varying security checks against the addresses or pointers.
The insight behind this approach is that if addresses or pointers are augmented with metadata, security checks can be automatically performed during runtime as a function of the metadata with the addresses or pointers.

Tamperable metadata augmentation based defenses maintain their metadata where the integrity of the metadata cannot be enforced. For example, \cite{stackguard_canaries}
maintains its metadata on the stack and \cite{qualcomm_white_paper, armmte, aos, c3, no-fat} maintain their metadata inside unused upper bits of pointers. Since these locations can be overwritten by a memory corruption exploit, tamperable metadata augmentation based defenses can also be categorized among mitigations that perform spoofable security checks. To mitigate possible spoofing attempts, tamperable metadata augmentation based defenses maintain the metadata as a secret that is private to their security domain and with high entropy.
Thus, if an attacker can leak this secret metadata from the victim's security domain, then the attacker can next perform a memory corruption attack while utilizing this leaked secret metadata to spoof security check(s) performed.
Examples of such defenses include Stack Smashing Protection~\cite{stackguard_canaries}, ARM Pointer Authentication (PA)~\cite{qualcomm_white_paper}, ARM Memory Tagging Extension (MTE)~\cite{armmte}, Always On Heap Memory Safety (AOS)~\cite{aos}, Cryptographic Capability Computing (C3)~\cite{c3}, and No-FAT~\cite{no-fat}.
\joel{No-FAT is listed as both tamperable and non-tamperable?}

\paragraph{Tamperproof Metadata Augmentation}
Tamperproof metadata augmentation based defenses similarly augment addresses or pointers with metadata that is used to perform varying security checks. 
The difference lies in the fact that instead of relying on privacy and high entropy of the metadata, these defenses directly enforce integrity of their metadata by other means. 

Today, there exists three varying approaches for enforcing metadata integrity. First, mitigations that perform out-of-bound security check for all memory accesses can place the metadata in an area outside the bounds of any other object in the address space called \emph{shadow memory}~\cite{intelmpx, hardbound, watchdog, watchdoglite, chex86}. Alternatively, mitigations can transparently tag the memory addresses that store the metadata by leveraging additional specialized hardware called \emph{tagged memory}~\cite{cheri, zero, rest}. Lastly, mitigations can leverage \emph{page attributes} to enforce integrity of the pages that hold the metadata, as in \cite{intelcet, armbti}.

Since the metadata which is used to perform security checks cannot be modified by an attacker, the security checks that are performed by these defenses cannot spoofed. As such, these defenses are unspoofable and thus are not vulnerable to \ssb attacks. Examples of such defenses include CHERI~\cite{cheri}, Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog}, WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86}, No-FAT~\cite{no-fat}, Intel CET~\cite{intelcet}, ARM BTI~\cite{armbti}, ZERO~\cite{zero}, REST~\cite{rest}, and Califorms~\cite{califorms}.

\begin{comment}
At a high level, when focusing on \ssb attacks, memory corruption mitigations can first be divided into two major categories depending on how whether additional security information 1) augments addresses separately or 2) is directly entangled with the addresses. 
\emph{Address augmentation} based defenses augment pointers (i.e., addresses) with additional information called ``\emph{metadata}'' that is maintained separately from the pointers. %This additional information is later used to perform additional security checks when the pointer is used. 
%We call such augmented information that is maintained separately ``metadata''. 
On the other hand, \emph{address layout randomization} based defenses  add random ``\emph{offsets}'' to the address of the various (sub-)objects, entangling these offsets with the originally predictable (sub-)object addresses. 
Hence, this first classification allows one to recognize whether 
%Notably, unlike ``metadata'' which is maintained separately from objects in memory for address augmentation based defenses, these ``offsets'' or ``deltas'' become entangled with the location of objects in the address space. 

For address augmentation based defenses, we further subdivide them depending on whether the augmented metadata is 1) \emph{tamperable} (i.e, modifiable) or 2) \emph{tamperproof} (i.e., not modifiable) in the presence of an attacker-controlled memory-write vulnerability. 
We do not subdivide address layout randomization based defenses because, in the presence of an attacker-controlled memory-write vulnerability, a pointer being overwritten is always entangled with the offset. In other words, for address layout randomization based schemes, the added offsets are inevitably always tamperable. We 

This two-level classification is useful in studying the security of these defenses against \ssb attacks for two reasons: 1) It allows 

\paragraph{address augmentation vs address layout randomization}
\paragraph{tamperable vs tamperproof}
- tamperable, but private + high entropy (i.e., info=secret). <- hence may be vulnerable to information disclosure
- tamperproof: public (i.e., info not secret), but protected from integrity attacks. <- hence not vulnerable to information disclosure 
\paragraph{tamperp}

\begin{footnotesize}
\begin{verbatim}
- maybe just write about each category now...
- tamperable defenses need to make it hard for an attacker
  to forge rouge metadata/offset -> high entropy + privacy
    -> they become especially vulnerable towards 
       information disclosure attacks.
       (hence vulnerable to side-channel attacks)
- tamperproof does not need to worry about forging rouge metadata
  - in fact, all defenses that are tamperproof maintain 
    public metadata (e.g., base/bound, endbranch, 
    location of redzones).
\end{verbatim}
\end{footnotesize}


\asplosdel{
In this paper, we study state-of-the-art
%In this paper, we study currently-deployed, and next-generation 
%\mengjia{I tend to use "next-generation" as a positive word to advocate something. Can we find a less positive word?} 
memory corruption mitigation proposals, from both academia\hbox{~\cite{hardbound, watchdog, watchdoglite, aos, chex86, califorms, rest, morpheus, cheri, no-fat,zero,c3, usenix_aslr}} and industry\hbox{~\cite{intelmpx, armmte,intelcet,armbti, armpa, pax_aslr}}, with a focus on hardware-software co-design proposals.
%In particular, we focus on the security of the defense proposals against exploits that target the synergies between memory corruption ~\cite{jop, schuster2015counterfeit, shacham2007geometry, brop} and side channel~\cite{spectre, meltdown} attacks. 
%\mengjia{removed last sentence... seems a bit repetitive. ok?}
%\weon{yep}
%\mengjia{what does this sentence mean? strength?}\weon{changed to security. can also say resilience.}
Our goal is to identify and analyze a meaningful subset of the common weaknesses in memory corruption mitigations that may be exploited due to the presence of side-channel vulnerabilities in modern processors.
%\subsection{Taxonomy}
%\label{sec:taxonomy}
%\blfootnote{\textsuperscript{$\dagger$}Califorms maintains tamperproof metadata for adjacent vulnerability protection and adds randomness to the size of the metadata for non-adjacent vulnerability protection; the randomness regarding the size of the metadata is vulnerable to information disclosure attacks.} 
%\blfootnote{\textsuperscript{$\ddagger$}No-FAT maintains tamperproof metadata for spatial protection, but tamperable metadata for temporal protection; the tamperable metadata is vulnerable to information disclosure attacks.}
%\mengjia{TODO: this paragraph could be moved later or to the begining of S3.2. We can decide later.}
%To better anticipate this security crisis, we perform a systematic analysis of state-of-the-art memory corruption defenses.
%, with a synergistic threat model, considering both memory corruption vulnerabilities in the software and side-channel vulnerabilities in the hardware.
%Given the vast number of mitigation mechanisms, we start by creating a taxonomy with a focus on analyzing whether a mitigation mechanism can be bypassed when assisted with information leakage attacks.
Given the vast number of mitigation mechanisms, we start by creating a taxonomy. The taxonomy focuses on analyzing whether a memory corruption mitigation mechanism can be penetrated or bypassed, by performing information leakage attacks using micro-architectural side-channels in the hardware.
}

%We find many defenses to be broken in the presence of a synergistic threat model. Furthermore, in \cref{attackvector}, we find that many defenses break due to the leakage of the micro-architectural side-effects, which can be leaked through side-channels on the hardware, but cannot be observed by secondary software vulnerabilities such as out-of-bound reads.
%To identify memory corruption mitigations which are potentially vulnerable to synergistic attacks, we must first create abstraction levels in which we can reason about their security properties against such threats. In this subsection, we build abstractions from fundamental properties that lead to (or protect from) vulnerabilities in the memory corruption defense proposals against synergistic attacks. We will base our discussion of the mitigation schemes, and their security, on these abstractions. 

\asplosdel{
We show our taxonomy in \hbox{\cref{fig:taxonomy}}  with examples of mitigation mechanisms for each category.
The highlighted mechanisms are vulnerable to information disclosure attacks.
%\mengjia{say we highlight the ones are vulnerble}
At a high level, memory corruption mitigations use two major strategies, i.e., \emph{address augmentation} and \emph{address layout randomization}.
%\mengjia{todo: can we change to "management" or something else, otherwise it is so close to ASLR} \weon{i prefer randomization (because what they do is randomization). note that its not just ASLR -- there's instruction set randomization etc. i feel like management is too abstract.}


%Address augmentation mechanisms try to augment pointers (i.e., addresses) with extra information when creating a pointer and perform a security check when using the pointer.
Address augmentation mechanisms try to augment pointers (i.e., addresses) with additional information regarding the pointer when creating a pointer, and later perform a security check when the pointer is used.
We call the augmented information ``\emph{metadata}''.
%Depending on whether the metadata is modifiable or tamperable by the adversary, we further classify these metadata into two sub-categories,
Depending on whether the metadata is modifiable by an adversary, we further classify these metadata into two sub-categories:
\textit{tamperproof} metadata and \textit{tamperable} metadata.
}

%Figure \ref{fig:flowchart} shows the different abstractions of memory corruption mitigations, systematised into a taxonomy.
%A defense proposal may either \textit{augment} each memory address with some \textit{metadata} to check whether a memory access is a legal, or \textit{randomize} the layout of different regions of the address space, to obfuscate the run-time addresses of the gadgets. In the taxonomy, we further divide the address augmentation mitigations on whether their metadata is \textit{tamperproof} or \textit{tamperable}. Defense proposals which incorporate tamperproof metadata can be abstracted into defenses which maintain \textit{full information} or \textit{partial information}. 

%Tamperproof \mengjia{metadata} defense proposals which maintain full information, augment every memory access with metadata indicating \textit{base} and \textit{bound} of each access for spatial safety and/or \textit{identifier} for temporal safety. Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog}, WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86}, and No-FAT~\cite{no-fat} maintain this metadata in a shadow space outside the base and bounds of any userspace objects. Hence, their defense proposal is able to comprehensively protect the metadata from software vulnerabilities such as arbitrary writes. CHERI~\cite{cheri} also maintains the base and bounds metadata, but instead of placing its metadata inside a safe shadow space, it inlines the metadata into all pointers (called fat pointers). To enforce the integrity of its metadata, CHERI utilizes an additional feature called tagged memory to tag its metadata for integrity checks. 
%Despite the high security guarantee of this class of defense proposals, they come with expensive performance and energy overheads due to the excessive data movement and storage incurred by maintaining such a large amount of metadata.


%In the case where the metadata is tamperproof, the metadata content is generally public. For example, the mitigation mechanism could maintain the full information for each pointer including the base and bound information for spatial safety and allocation identifier for temporal safety, such as CHERI~\cite{cheri}, Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog}, WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86}, and No-FAT~\cite{no-fat}~\footnote{xxx}.

%However, these mechanisms usually come with expensive performance and energy overheads due to the excessive metadata accesses, as well as storage overhead incurred by maintaining a large amount of metadata.

\paragraph{Tamperproof metadata}
Tamperproof metadata defense schemes which maintain full information sustain and operate on the full information of each pointer such as the base and bound of the pointer for spatial safety or an allocation identifier for temporal safety.
\weon{trim?}
Examples of such defense proposals include CHERI~\cite{cheri}, Intel MPX~\cite{intelmpx}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog}, WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86}, and No-FAT~\cite{no-fat}.
To ensure the metadata is tamperproof, these mechanisms either maintain the metadata in shadow space or leverage additional hardware tagging mechanism.
Despite providing full memory safety, these mechanisms come with expensive performance and energy overheads due to the excessive metadata accesses, as well as storage overhead incurred by maintaining a large amount of metadata.

%To address these overhead, researchers reduce the metadata size by replacing full pointer information with partial information to trade-off between performance and protection coverage, such as Intel CET~\cite{intelcet}, ARM BTI~\cite{armbti}, ZERO~\cite{zero}, REST~\cite{rest}, and Califorms~\cite{califorms}~\footnote{.... say }.
To address these overhead, researchers have proposed reducing the metadata size by replacing full information with partial information, trading-off protection coverage for performance. 
\weon{trim?}
Examples of such schemes include Intel CET~\cite{intelcet}, ARM BTI~\cite{armbti}, ZERO~\cite{zero}, REST~\cite{rest}, and Califorms~\cite{califorms}.
With partial information, these schemes offer a reduced protection coverage compared to those maintaining full information. 
%\yuheng{What is partial? if full infomation is (base, bound), is partial something like (last 12 bit of base, bound)? and what is protection coverage?}
%\mengjia{cut the example and cut the last sentence.}






%Tamperproof defense proposals which maintain partial information, augment a subset of memory accesses with lightweight metadata, providing much more ideal performance compared to defenses maintaining full information. Unlike mitigations which maintain full information, defenses which maintain partial information are diverse in their security goals, and as such, there exists a large variety in defining, maintaining and utilizing metadata. 
%For example, Intel CET~\cite{intelcet} Indirect Branch Tracking (IBT) uses \texttt{endbranch} instructions as its metadata. Intel CET-IBT marks valid branch target locations with an \texttt{endbranch} instruction, and the instruction after a branch is checked in the hardware to confirm that it is an \texttt{endbranch} instruction. 
%Intel CET~\cite{intelcet} Shadow Stack (SS) leverages the return addresses as its metadata. Intel CET-SS maintains a second stack in a shadow region of the memory that pushes the return addresses to the shadow stack on \texttt{call}s  and pops the return addresses off the shadow stack on \texttt{ret}s. 
%ZERO~\cite{zero}, REST~\cite{rest}, and Califorms~\cite{califorms} utilize tagged memory to enforce track their metadata. 
%ZERO~\cite{zero} implicitly tags each memory address in the microarchitecture with 2 bits, to mark an address among four different types: data, return adress, data pointer, and function pointer. ZERO enforces pointer integrity by blocking addresses of different types from overwriting another. 
%REST~\cite{rest} and Califorms~\cite{califorms} implicitly tags each memory address in the microarchitecture to blacklist memory addresses surrounding allocated objects. By doing so, REST and Califorms provides spatial safety against adjacent buffer overflows.

%These defense proposals which leverage only partial information, are also able to cheaply enforce the integrity of their metadata. Intel CET-IBT blocks adversaries from forging rogue \texttt{endbranch} instructions by enforcing W $\oplus$ X to code pages. Intel CET-SS protects the integrity of the shadow stack by extending page table protection with additional attributes. ZERO, REST, and Califorms metadata cannot be modified as the tags are managed implicitly by the micro-architecture.

%Despite the tamperproof property, as well as the low overhead of these defenses, the defenses leveraging partial information lack in the security they are able to provide.
%Intel CET-SS is able to mitigate ROP attacks, but lacks any protection against JOP attacks. 
%Intel CET-IBT narrows the attack vector of ROP and JOP attacks by limiting the branch target locations, but does fully mitigate these attacks. 
%ZERO provides pointer integrity, but is vulnerable to data corruption attacks. 
%REST is able to protect against adjacent buffer overflows, but provides no protection against non-adjacent buffer overflows. 
%Califorms provides protection against non-adjacent buffer overflows, by randomizing the size of the security bytes (i.e., blacklisted addresses), but we find that Califorms is vulnerable to synergistic attacks for non-adjacent buffer overflows. (\cref{attackvector}).


%Defenses which maintain partial information are diverse in their security goals, and as such, there exists a large variety in defining, maintaining and utilizing metadata.
Defenses which maintain partial information are diverse in their security goals, and as such, there exists a large variety of schemes in defining, maintaining and utilizing their metadata. %We defer the detailed discussion of each scheme to Appendix\mengjia{todo}, and only give one example to show that maintaining partial information can result in limited protection coverage.
%We defer the detailed discussion of each scheme to \cref{appendix:partial}, and discuss one example to explain the limited protection coverage provided by schemes maintaining partial information.
Due to space, we discuss one example here to explain the limited protection coverage provided by schemes maintaining partial information.
%For example, Intel CET~\cite{intelcet} offers indirect branch tracking to defend against jump-oriented programming (JOP)~\cite{bletsch2011jop}.
%\weon{After thinking, I think IBT is a better example than SS because SS's vulnerability is JOPs which IBT protects against. So, can't just say SS is weak, because you can argue there is also IBT}
\mengjia{Joel did not get this example.... }
\weon{Well, not sure if there's any better example... We can take it out entirely too...}
Consider Intel CET~\cite{intelcet}, which offers indirect branch tracking (IBT) to defend against jump-oriented programming (JOP)~\cite{bletsch2011jop}.
%Specifically, it introduces a new instruction \texttt{endbranch} to mark valid indirect call/jump targets in the protected program, and the hardware checks whether call/jump instructions transfer the control flow to one of the valid targets.
Specifically, IBT of Intel CET introduces a new instruction \texttt{endbranch} as metadata to mark valid indirect call/jump targets in the protected program, and utilizes the hardware to check whether a call/jump instruction transfers the control flow to one of the valid targets.
%Despite being highly effective, Intel CET cannot achieve context-sensitive control-flow integrity~\cite{criswell2014kcofi, abadi2009control, evans2015control} and can still be bypassed by advanced block-oriented programming~\cite{ispoglou2018block}.
Despite its efficacy, Intel CET does not achieve context-sensitive control-flow integrity~\cite{criswell2014kcofi, abadi2009control} and can broken by advanced block-oriented programming~\cite{ispoglou2018block}. \pwd{You may want to hammer home that this is solely b/c of the partial information conundrum} \yuheng{It seems this last sentence is explaining what "partial information" means. But I do not understand "context-sensitive control-flow integrity", an example on it?}

\paragraph{Tamperable metadata}
%To address the limited security coverage of defense mechanisms leveraging metadata with partial information, 
To achieve overall better trade-off in performance and security,
researchers in both academia~\cite{aos, c3, no-fat} and industry~\cite{armmte, sparc_adi, stackguard_canaries, armpa} have also begun extensively exploring tamperable metadata to provide similar security coverage at low performance overhead. 
%\yuheng{So we are using full information here?}
\weon{trim?}
Examples of such schemes include ARM Pointer Authentication (PA)~\cite{qualcomm_white_paper}, ARM Memory Tagging Extension (MTE)~\cite{armmte}, SPARC Application Data Integrity (ADI)~\cite{sparc_adi}, Always-On memory Safety (AOS)~\cite{aos}, Cryptographic Capability Computing (C3)~\cite{c3}, stack smashing protection~\cite{stackguard_canaries}, and No-FAT~\footnote{No-FAT generates a random number as a temporal id for an allocated object and stores the temporal id at the unused high bits of the pointer. Thus, when used for temporal safety, No-FAT's metadata is tamperable.}~\cite{no-fat}.
%In addition to maintaining tamperproof metadata, both the industry and academia have been extensively exploring another direction to combat memory corruption attacks via maintaining tamperable metadata, such as ARM Pointer Authentication (PA)~\cite{qualcomm_white_paper}, AOS~\cite{aos}, Intel Cryptographic Capability Computing (C3)~\cite{c3}, ARM Memory Tagging Extension (MTE)~\cite{armmte}, SPARC Application Data Integrity (ADI)~\cite{adi?}, stack canaries~\cite{stackguard_canaries}, and No-FAT~\footnote{No-FAT generates a random number as a temporal id for an allocated object and stores the temporal id at the unused high bits of the pointer. Thus, when used for temporal safety, No-FAT's metadata is tamperable.}~\cite{no-fat}.

%instead of relying on its entropy. Moreover, the security of these defense proposals tend to be independent to the confidentiality of the metadata. In many of these proposals, the metadata is usually already be public, dissipating the necessity of enforcing the privacy of the metadata.
%On the other hand, defense proposals which incorporate tamperable metadata allow direct modifications to the metadata. For example, ARM Pointer Authentication (PA), directly embeds the MAC of the pointer address as metadata inside the upper unused bits of the original address. Hence, the metadata is directly modifiable. 
%However, the metadata usually has high entropy and is normally private to the victim. The crux of these defense proposals is that the entropy of these metadata are too high to brute-force and leakage of the confidential metadata is blocked by the respective proposal.

%These schemes all share the common insight that the actual address space in a 64-bit architecture is usually less than 64 bits, resulting in 11-17 unused bits in a pointer which can be used to store metadata avoiding any storage overhead.
Except stack smashing protection~\cite{stackguard_canaries}, all these schemes leverage the common insight that the virtual address space in a 64-bit architecture is under-utilized in today's systems, resulting in 11-17 bits to be unused inside a pointer. This insight can be leveraged to store metadata into the unused bits of the pointer, avoiding storage overhead and transparently propagating the metadata with the pointer at no additional cost.
%On the other hand, defense proposals which incorporate tamperable metadata allow direct modifications to the metadata. For example, ARM Pointer Authentication (PA), directly embeds the MAC of the pointer address as metadata inside the upper unused bits of the original address. Hence, the metadata is directly modifiable. 
%However, the metadata usually has high entropy and is normally private to the victim. The crux of these defense proposals is that the entropy of these metadata are too high to brute-force and leakage of the confidential metadata is blocked by the respective proposal.

However, these schemes lead to a possible vulnerability as embedding the metadata inside the unused bits of the pointer allows the adversary to modify the metadata directly, possibly forging rogue metadata. 
To protect against this vulnerability, tamperable mitigation schemes enforce confidentiality of the metadata in its protection domain. 
%\yuheng{I feel a little weird to call this confidentiality. Because you are not simply hide the metadata, you are hiding how attack can generate a pac for a chosen address.}
The hope is that even if an adversary is able to forge the correct pointer, the adversary does not have the capability to forge the associated metadata to match the new forged pointer.
%The idea is that if an adversary attempts to modify the pointer value, in order to successfully bypass the protection mechanism, the adversary needs to additionally also modify the associated metadata to match the new pointer value.
Hence,  for these defense proposals to work, the key is to block any leakage of the confidential metadata, and maintain high entropy for these metadata to block brute-forcing.
%\mengjia{you should talk about that the attacker needs to forge the metadata, then talk about entropy and brute-force stuff. The logic in the last two sentences is not good.}

%Since the metadata is tamperable, these mitigation mechanisms try to achieve security by leveraging the confidentiality of the metadata.
%To protect against this vulnerability, these mitigation mechanisms try to achieve security by leveraging the confidentiality of the metadata.
%The idea is that if an adversary attempts to modify the pointer value, in order to successfully bypass the protection mechanism, the adversary needs to additionally also modify the associated metadata to match the new pointer value.
%If the metadata does not match the new pointer value, a suspicious event is detected and generally, the program will crash.
%However, these schemes work by heavily relying on the confidentiality of the metadata and can become completely ineffective if the metadata values are leaked.

There are two types of tamperable metadata with a varying amount of entropy. 
The first type of metadata is generated using some form of cryptographic function of the pointer value.
\weon{trim?}
For example, the metadata in ARM PA~\cite{qualcomm_white_paper} and AOS~\cite{aos} is a cryptographic hash of the pointer value generated using the QARMA algorithm~\cite{avanzi2017qarma}.
The metadata in C3~\cite{c3} is a cryptographic address generated from the virtual address of the pointer value using K-Cipher~\cite{kcipher}.
%to generate a cryptographic hash of the pointer value, and modifying the pointer value will result in a mismatch of the cryptographic hash.
%Alternatively, Intel C3~\cite{c3} generates a unique and distinct cryptographic address for each allocated memory space.
%If a cryptographic address is tampered, the decrypted plaintext address will be garbled.
The second type of metadata uses random numbers, as in the memory tags in ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi}, canaries used for stack smashing protection~\cite{stackguard_canaries}, and the tag used for temporal safety in No-FAT~\cite{no-fat}.

%There are two types of tamperable metadata with a varied amount of entropy.
%The first type of metadata is generated using some form of cryptographic function of the pointer value.
%For example, the metadata in ARM PA~\cite{qualcomm_white_paper} and AOS~\cite{aos} is a cryptographic hash of the pointer value generated using the QARMA algorithm~\cite{avanzi2017qarma}.
%The metadata in Intel C3~\cite{c3} is the cryptographic address generated for each allocated memory space. We elaborate more on the design details of C3 in \cref{sec:poc3}.
%to generate a cryptographic hash of the pointer value, and modifying the pointer value will result in a mismatch of the cryptographic hash.
%Alternatively, Intel C3~\cite{c3} generates a unique and distinct cryptographic address for each allocated memory space.
%If a cryptographic address is tampered, the decrypted plaintext address will be garbled.
%The second type of metadata uses random numbers, such as stack canaries~\cite{stackguard_canaries}, the memory tag in ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi}, and the tag used for temporal safety in No-FAT~\cite{no-fat}.



\paragraph{Address layout randomization}
The key idea of address layout randomization schemes is to randomize the position of objects in virtual memory.
\weon{trim?}
Examples of such schemes include ASLR~\cite{aslr-ng, canella2020kaslr, kaslr_lwn, pax_aslr, usenix_aslr}, Califorms~\cite{califorms}, and Morpheus~\cite{morpheus}.
%The idea of address layout randomization is to randomly arrange the position of code and data memory regions. such as ASLR~\cite{aslr-ng, canella2020kaslr, kaslr_lwn, pax_aslr, usenix_aslr}, Califorms~\cite{califorms}, and Morpheus~\cite{morpheus}.

The insight behind this type of mitigations is that if the address of the gadgets (used in ROP/JOP attacks) in the virtual memory is not fixed, the adversary is unable to divert the control flow reliably.
%As discussed in detail in \cref{sec:motivate}, 
\weon{trim?}
ASLR~\cite{pax_aslr, usenix_aslr} randomizes the segment offsets added to the memory segments once at the beginning of the program.
\weon{trim?}
Morpheus~\cite{morpheus} periodically re-randomizes the segment offsets using additional hardware features.
\weon{trim?}
Califorms~\cite{califorms} randomizes the size of the blacklisted regions in memory.
%, augmenting partial-info metadata techniques with address layout randomization techniques.
%\mengjia{I cut some text since it sounds confusing...}
However, as discussed in \cref{sec:motivate}, this category of mitigations can be broken if information regarding the layout can be acquired using information leakage attacks.
%Morpheus~\cite{morpheus} periodically re-randomizes the offset.
%Califorms~\cite{califorms} additionally incorporates address blacklisting~\cite{...} with address layout randomization.
%However, as discussed in \cref{sec:motivate}, mitigations in this category can be bypassed if the layout can be recovered via information leakage attack.
\end{comment}


\paragraph{Taxonomy summary}
In this section, we have systematized a taxonomy of state-of-the-art memory corruption defenses focusing on their security against \ssb attacks. 
In this taxonomy, two categories of defenses (in red in \cref{fig:taxonomy}) may be vulnerable to \ssb attacks. 
Specifically, mitigations that augment tamperable metadata or add random offsets to addresses or pointers inevitably perform spoofable security checks; these spoofable security checks make these defenses sensitive to information disclosure attacks, since the leakage of secret metadata or offset empowers an adversary with the ability to disarm a security check and ultimately bypass the respective defenses.
On the other hand, the taxonomy has also led to finding of a class of defenses that are resilient to \ssb attacks; such defenses enforce the integrity of their metadata by techniques such as out-of-bound shadow memory, tagged memory, or page attributes. Furthermore, the metadata of these defenses are generally public information and indifferent to information disclosure. 

Based on this taxonomy, we systematically categorized 20 defenses.
%The insights of our taxonomy led to 10 possibly vulnerable defense findings, among the 20 studied in this paper.\mengjia{this sentence is a bit confusing, because the readers does not know what these mechanisms are vulnerable to, so they cannot appreciate the number 10, since they do no have the context yet.}
%Our taxonomy is insightful in helping figure out which mitigation mechanisms are vulnerable to information disclosure attacks.
The nature of our taxonomy allowed us to easily identify possible vulnerabilities
leading to the discovery of 10 possibly vulnerable defenses, among which 5 are
either currently deployed, or soon to-be deployed in products by the industry. 
We believe our taxonomy is valuable for identifying future memory corruption defenses vulnerable to \ssb attacks.

In \cref{sec:model}, we analyze how side-channel vulnerabilities can be exploited during the first step of an \ssb attack, to leak the secrets from the 10 defenses that perform spoofable security checks.


\begin{comment}
%\mengjia{there exists some issue with the ordering of these sentences. My suggestion:
%1. we should first give analysis results, the result is not the number of vulnerable schemes, the result should be which *categories* are vulnerable to what *attacks*,
%2. then talk about the number of vulnerable mitigations in this analysis}
In this section, we have systematized a taxonomy of the state-of-the-art memory corruption defenses.
%focusing on hardware-software co-design solutions.
In our taxonomy, we found two categories of mitigations (highlighted in \cref{tab:taxonomy}) that may be vulnerable to synergistic attacks. 
Specifically, mitigations that leverage tamperable metadata can be broken if the metadata is leaked, and defenses via address layout randomization can be broken if the randomized offsets are leaked. 
\mengjia{highlight key takeaways. I think I want to figure out why these two schemes are vulnerable to information leakage attacks. Even though they are both vulnerable, the stuff attackers can modify is different.\\
Also a good point to sumamrize why the others are not vulnerable.}

Based on this taxonomy, we systematically categorized 20 defenses.
%The insights of our taxonomy led to 10 possibly vulnerable defense findings, among the 20 studied in this paper.\mengjia{this sentence is a bit confusing, because the readers does not know what these mechanisms are vulnerable to, so they cannot appreciate the number 10, since they do no have the context yet.}
%Our taxonomy is insightful in helping figure out which mitigation mechanisms are vulnerable to information disclosure attacks.
The extensive nature of our taxonomy allowed us to easily identify possible vulnerabilities
leading to the discovery of 10 possibly vulnerable defenses, among which 5 are
either currently deployed, or soon to-be deployed in products by the industry. 
%\pwd{Is there a particular pattern which dicates which schemes are insecure/secure?} \pwd{ah ok, it's the highlighted entries -- you should probably emphasize that in the text (in addition to the figure caption)}
%Specifically, we find that mitigation mechanisms that leverage tamperable metadata can be bypassed if the metadata is leaked, and mechanisms using address layout randomization can be bypassed if the randomized offsets are leaked.
We believe our taxonomy is valuable to understanding the possible vulnerabilities of future defense mechanisms.

In the rest of this paper, we focus our synergistic attack analysis on these two mitigation categories, i.e., the 10 possibly vulnerable mitigation examples.
%found in our the taxonomy.
%Therefore, we focus our synergistic attack analysis on these two mitigation categories, which include 10 mitigation examples.
%We think it is promising to use this taxonomy to understand the vulnerability of future mitigation mechanisms.

%Moreover, it is promising the use our taxonomy to analyze future mitigation mechanisms.
%To summarize our analysis, we find that since mitigation mechanisms that leverage tamperable metadata or address layout randomization are likely to be bypassed by 


%\paragraph{Goal: Analysis of memory corruption mitigations that are vulnerable to information disclosure attacks (\cref{fig:flowchart})} 
%As shown in \cref{fig:flowchart}, there exists a common set of techniques among memory corruption mitigations that incorporate tamperable metadata or randomize the address layout. 

%\mengjia{it is better to follow the diagram... so i would prefer to either change the diagram or postpone the discussion on address randomization}
%This classification is insightful in regards to the security of the defense proposal.
%For example, if the defense proposal augments each accessed memory address with a random number as metadata (that is later verified), the confidentiality of this metadata is integral to the integrity of the system. 
%On the other hand, if the the defense proposal randomizes the address space layout, the randomized offset of the code and data sections is integral to the integrity of the system. 
%\mengjia{"integral to the integrity of the system" is a bit confusing. }
%In both cases, the goal of the attacker is to leak some secret of the defense proposal, whether it be some metadata or some offset. 
\end{comment}


==> sections/bac-history-memorycorruption.tex <==

\subsection{History of Memory Corruption Attacks and Mitigations}
\label{sec:bac_history}
%\vspace{+2ex}


\mengjia{my feedback for this subsection is that, we do not need to talk about the history. I feel code injection is such an old thing, which does not exist mostly, but we spend a lot of text on that, which is not necessary. \\
A very important thing is that the background is used to serve for the main content, and define some terminologies that will be used later. If you define something that will not be used, then that is not a good use of space.\\
Let me suggest something as follows. \\
1. memory corruption -> software bugs, such as buffer overflow, use-after-free, non-adjacent memory write\\
*** IMPORTANT: provide code snippet if possible, because we will use non-adjacent memory write
2. with the bug, one can do control-flow hijacking by 1) directly introduce payload; 2) ROP/JOP, and say ROP/JOP are the main threats nowadays; or they can leak secret data, such as heartbleed.\\
3. Then talk about mitigations: introduce the term for spatial memory safety and temporal memory safety\\
4. (very brief, just mention defense names) then other practical mitigations include stack canary, ASLR, pointer integrity, .... and refer to the SoK paper}


Memory corruption bugs are an orthogonal class of vulnerabilities with a long history of exploits. Applications written in low-level languages like C or C++ are prone to memory corruption bugs. For instance, a vulnerable program may read data over a network into a buffer lacking sufficient bounds checking, overwriting memory beyond the end of the buffer. Consequentially, return addresses and function pointers may be tampered, manipulating the program's control-flow and eventually leading control hi-jack. 

In the early days of the attack on memory, it was common for an attacker to include the malicious code inside the \textit{payload} and overflow a buffer on the stack. This allowed the attacker to point the overwritten return address to a known address on the stack, where the malicious code resides~\cite{phrack-stacksmashing}.

Fortunately, such \textit{code injection} attacks are no longer practical on all modern systems, as contemporary processors and operating systems transparently provide a defense known as \textit{non-executable memory}, where they cooperatively mark the data memory pages as non-executable.

To defeat the defense provided by non-executable memory, a technique known as \textit{return-to-libc} was developed. To bypass the step of including the malicious code inside the payload, the attacker reuses a high-level library function as the return address. In particular, in \cite{return-to-libc1997}, the authors return to the \texttt{system()} function, with only a single argument passed on the stack, and run arbitrary shell code.

More versatile attacks such as \textit{return-oriented programming}, or ROP, were also developed. In ROP, the attacker reuses code-snippets (called \textit{gadgets}) inside the program's address space, instead of high-level functions. Such gadgets are put together to perform arbitrary computation without the reliance on injected code~\cite{rop2012}.

Defense researchers were quick to respond. \textit{Stack smashing protection} was soon introduced as an additional defense against memory corruption attacks. By placing a random value (called \textit{canary}) between the saved return address and buffers on the stack during function prologue, the integrity of the saved return address is later checked at the function epilogue, before the return of the function~\cite{stackguard}.

\textit{Address space layout randomization}, or ASLR, was also introduced as another defense against memory corruption vulnerabilities. ASLR randomizes the location of memory segments, such as code and data, and thus the attacker cannot know the location of the gadget he or she wants to reuse~\cite{pax_aslr, usenix_aslr}.

The defense arsenal accumulated in modern systems create a major challenge for attackers. However, stack smashing detection and ASLR have been shown to be defeatable through \textbf{additional vulnerabilities that \textit{leak information} about the secret}. Format string vulnerabilities have been demonstrated to leak information about the randomized value of the canary on the stack, and the randomized address locations of the code in the program's address space~\cite{phrack-formatstring}. Previous attacks have also demonstrated the feasibility of brute-forcing the canary~\cite{brop}, or the address layout~\cite{aslr32break, brop} in crash-resistant programs.


==> sections/backup.tex <==
%\begin{figure*}[t]
%    \centering
%    \includegraphics[width=0.8\textwidth]{figures/table-assets.png}
%    \caption{\rev{Memory Corruption Exploit Mitigation}}
%    \label{tab:assets}
%\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{comment}

\begin{table*}[t]
\footnotesize
\begin{center}
\begin{tabular}{|l|l|llll|l|l|l|}
\hline
\multirow{2}{*}{Classification} &
  \multirow{2}{*}{Proposal} &
  \multicolumn{4}{l|}{Protected Assets} &
  \multirow{2}{*}{Maturity} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Metadata\\ Overhead\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Performance \\ Overhead\end{tabular}} \\ \cline{3-6}
 &
   &
  \multicolumn{1}{l|}{RET} &
  \multicolumn{1}{l|}{Code Ptr} &
  \multicolumn{1}{l|}{Data Ptr} &
  Data &
   &
   &
   \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Tamperproof\\ Metadata\end{tabular}} &
  ARM BTI &
  x &
  x &
  x &
  x &
  Commercialized &
  1 instruction per branch target &
  $ \propto $ \# of branches \\
 &
  Intel CET &
  \checkmark &
  x &
  x &
  x &
  Commercialized &
  \begin{tabular}[c]{@{}l@{}}1 instruction per branch target,\\ 1 word per return address\end{tabular} &
  $ \propto $ \# of branches and returns \\
 &
  ZERO &
  \checkmark &
  \checkmark &
  \checkmark &
  \checkmark &
  Simulated &
  2 bits per word &
  $ \propto $ \# of mem accesses \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Address Layout\\ Randomization\end{tabular}} &
  ASLR &
  \checkmark &
  \checkmark &
  \checkmark &
  \checkmark &
  Commercialized &
  none &
  negligible \\
 &
  Morpheus &
  \checkmark &
  \checkmark &
  \checkmark &
  \checkmark &
  Simulated &
  2 bits per word &
  $ \propto $ 1/re-randomization interval \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Tamperable\\ Metadata\end{tabular}} &
  Stack Canary &
  \checkmark &
  x &
  x &
  x &
  Commercialized &
  8B per return address &
  $ \propto $ \# of returns \\
 &
  ARM PA &
  \checkmark &
  \checkmark &
  \checkmark &
  x &
  Commercialized &
  Embeded inside pointer &
  $ \propto $ \# of pointer derefs \\ \hline
\end{tabular}
\caption{\rev{Tradeoffs in Reactive Memory Safety Schemes}}
\label{tab:assets}
\end{center}
\end{table*}
\end{comment}

\begin{comment}

\begin{table*}[t]
\footnotesize
\begin{center}
\begin{tabular}{|c|c|cc|c|c|c|c|}
\hline
\multirow{2}{*}{Classification} &
  \multirow{2}{*}{Proposal} &
  \multicolumn{2}{c|}{Spatial Protection} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Temporal\\ Protection\end{tabular}} &
  \multirow{2}{*}{Maturity} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Metadata \\ Overhead\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Performance \\ Overhead\end{tabular}} \\ \cline{3-4}
 &
   &
  \multicolumn{1}{c|}{Inter-Object} &
  Intra-Object &
   &
   &
   &
   \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Tamperproof\\ Metadata\end{tabular}} &
  CHERI &
  \checkmark &
  \checkmark &
  x &
  Prototyped &
  256 bits per pointer &
  $ \propto $ \# of pointer ops \\
 &
  Intel MPX &
  \checkmark &
  \checkmark &
  x &
  \begin{tabular}[c]{@{}c@{}}Commercialized,\\ but discontinued\end{tabular} &
  2 words per pointer &
  $ \propto $ \# of pointer derefs \\
 &
  Hardbound &
  \checkmark &
  \checkmark &
  x &
  Simulated &
  \begin{tabular}[c]{@{}c@{}}0-2 words per pointer,\\ 4 bits per word\end{tabular} &
  $ \propto $ \# of pointer derefs \\
 &
  Watchdog &
  \checkmark &
  \checkmark &
  x &
  Simulated &
  4 words per pointer &
  $ \propto $ \# of pointer derefs \\
 &
  Watchdoglite &
  \checkmark &
  \checkmark &
  x &
  Simulated &
  4 words per pointer &
  $ \propto $ \# of pointer ops \\
 &
  CHEx86 &
  \checkmark &
  x &
  \checkmark &
  Simulated &
  2 words per pointer &
  $ \propto $ \# of pointer ops \\
 &
  REST &
  adjacent only &
  x &
  \checkmark &
  Simulated &
  8-64B token &
  $ \propto $ \# of mem accesses \\
 &
  Califorms &
  \checkmark &
  \checkmark &
  \checkmark &
  Simulated &
  1-7B per pointer &
  $ \propto $ \# of mem accesses \\
 &
  No-FAT &
  \checkmark &
  \checkmark &
  \checkmark &
  Simulated &
  1KB per process table &
  $ \propto $ \# of pointer derefs \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Tamperable\\ Metadata\end{tabular}} &
  ARM MTE &
  \checkmark &
  x &
  \checkmark &
  \begin{tabular}[c]{@{}c@{}}(To be) \\ commercialized\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Embed inside pointer and \\ 4 bits per 16B objects\end{tabular} &
  $ \propto $ \# of pointer derefs \\
 &
  SPARC ADI &
  \checkmark &
  x &
  \checkmark &
  Commercialized &
  \begin{tabular}[c]{@{}c@{}}Embed inside pointer and \\ 4 bits per 64B objects\end{tabular} &
  $ \propto $ \# of pointer derefs \\
 &
  AOS &
  \checkmark &
  x &
  \checkmark &
  Simulated &
  8B per pointer &
  $ \propto $ \# of pointer derefs \\
 &
  C3 &
  \checkmark &
  x &
  \checkmark &
  Simulated &
  Entangle with pointer &
  $ \propto $ \# of pointer derefs \\ \hline
\end{tabular}
\caption{\rev{Tradeoffs in Preactive Memory Safety Schemes}}
\label{tab:safety}
\end{center}
\end{table*}
\end{comment}


==> sections/intro-old.tex <==
\section{Introduction}
%\vspace{+2ex}


%\mengjia{TODO.... need to say it is not spectreRSB or SpecROP... It is very likely some people will think it in this way...
%explitictly say we conduct a code-reuse attack, not just to leak information....}

%\mengjia{we should say we analyzed xx mitigations, and found 10 are vulnerable to our synergistic attacks, among which xx are industry proposals which is currently being deployed or will be deployed in the future.}

%Memory corruption vulnerabilities~\cite{szekeres2013sok} are one of the oldest security problems in computer systems, which have existed for more than 30 years and still continue to widely affect modern software systems~\cite{roemer2012rop}.
%Having existed for over 30 years \pwd{awkward wording},

\weon{todo: fix  ordering of citation numbers}
Memory corruption bugs~\cite{szekeres2013sok}  are one of the oldest security problems in computer systems. %~\cite{roemer2012rop}.
%Today, memory corruption bugs continue to endanger modern systems~\cite{roemer2012rop}.
%According to the MITRE 2021 rankings~\cite{mitre}, the top 10 most dangerous software weaknesses include multiple memory corruption bugs, such as out-of-bound writes, out-of-bound read, and use-after-free.
According to the MITRE 2021 rankings~\cite{mitre}, the top 10 most dangerous software weaknesses encompass multiple memory corruption bugs, including out-of-bound writes, out-of-bound reads, and use-after-frees.

%It has been a critically important research area on how to design effective and low-overhead memory corruption mitigations~\cite{xxxx}.
%Extensive progress has been made in both academia and industry.
Designing effective and low-overhead \asplosdel{protection} \asplosrev{memory safety} mechanisms has become a rich research area~\cite{szekeres2013sok} and extensive progress has been made in both academia and industry.
%For example, in academia, there have been a vast number of works on leveraging architectural innovations to reduce performance and storage overhead of software mitigations, such as REST, ZERO, etc. ...\mengjia{list}.
For example, in academia, there have been a vast number of works proposing to leverage architectural innovations or insights to reduce performance and storage overhead of software-only defenses, 
including CHERI~\cite{cheri}, Hardbound~\cite{hardbound}, WatchDog~\cite{watchdog}, WatchdogLite~\cite{watchdoglite}, CHEx86~\cite{chex86}, No-FAT~\cite{no-fat}, ZERO~\cite{zero}, REST~\cite{rest}, Califorms~\cite{califorms}, AOS~\cite{aos},  C3~\cite{c3}, and Morpheus~\cite{morpheus}.
%Moreover, given the serioys security threats posed by memory corruption vulnerabilities, the industry has been actively adopting mitigation mechanisms and major processor vendors have announced and shipped products with features, such as Intel MPX~\cite{intelmpx}, Intel CET~\cite{intelcet}, ARM Pointer Authentication~\cite{armpa}, ARM MTE~\cite{armmte}, SPARC ADI~\cite{sparc_adi}.
Moreover, the industry has been actively adopting mitigation mechanisms. 
For example, major processor vendors have announced and shipped products with many features supporting increased memory safety, such as Intel MPX~\cite{intelmpx}, Intel CET~\cite{intelcet}, ARM Pointer Authentication~\cite{armpa}, ARM MTE~\cite{armmte}, and SPARC ADI~\cite{sparc_adi}.



% \begin{verbatim}

% - synergistic attack
%     - what it is at high level, with a simple example on aslr or pacman
%     - say why studying this is important
%         - across multiple layers of system and sit in intersections between threat models
%         - need expertise on both sides...
%     - SSB, this paper, one specific example
%         - leak secret in mitigations via side channel
%         - bypass mitigation using the leaked secret
% - strong motivation/challenges/limitations of existing work
%     - no other work looks at this problem systematically, mostly as a case study for side channel attack
%     - mitigations come in many different formats, how to model them and learn from that to develop countermeasure..
% - SSB
%     - define what SSB is
%     - taxonomy and modeling 
%     - summarize S5 and S6, potentially S8 (countermeasure)

% \end{verbatim}

















%\paragraph{Motivation: Synergistic Attacks}
%Even though a vast number of solutions have been proposed and deployed, memory corruption attacks continue to pose a serious threat.
Despite the vast number of solutions that have been proposed and deployed, memory corruption attacks continue to pose a serious security threat.
%Even worse, we observe that there is a trend of \emph{using synergistic attack strategies to bypass memory corruption mitigations}.
More concerningly, we observe that there is a growing trend of leveraging \emph{synergistic} attack strategies to bypass memory corruption mitigations. %\pwd{Wouldn't italicize this}.
%Specifically, instead of only exploiting memory corruption bugs, attackers build advanced attacks by \emph{combining} attack strategies from a very different threat model which target a different layer of the system. 
Specifically, instead of only exploiting memory corruption vulnerabilities, adversaries have started to build advanced attacks by \emph{combining} attack strategies which fall into traditionally disjoint threat models, targeting different layers of the system stack.
Notably, multiple recent works have demonstrated that microarchitectural side channels, which exploit \emph{hardware} vulnerabilities, can be used to break Address Space Layout Randomization (ASLR)~\cite{speculativeprobing, hund13, gras17} and ARM Pointer Authentication (PA)~\cite{pacman}, two primary defenses in modern systems for protecting against \emph{software} vulnerabilities.

\paragraph{Motivation: \attackname Attacks} We call an attack a \emph{\ssb} attack if it exploits microarchitectural side-channels to bypass software security mechanisms such as ASLR and ARM PA. Specifically, a \ssb attack exploits side-channels to leak some secret that is critical to the security of a memory corruption mitigation. Once a speculative shield bypass attack acquires the secret knowledge necessary to bypass the mitigation mechanisms, it utilizes this knowledge to conduct a memory corruption exploit, such as control-flow hijacking.

It is critically important to study \ssb attacks.
On one hand, \ssb attacks out-perform traditional memory corruption attacks, violating both confidentiality and integrity of the system in ways that were not traditionally possible.
On the other hand, \ssb attacks are easy to miss and difficult to mitigate.
Modern systems have a large and complex attack surface.
To handle such non-trivial complexity, security researchers today often partition the problem space into disjoint threat models, exploring each threat model separately. 
However, to mitigate against \ssb attacks, researchers must first acquire domain expertise that spans both side-channel vulnerabilties as well as memory corruption vulnerabilities.

\paragraph{This Paper}
We strive to provide the \emph{first} systematic analysis of one such threat model; a threat model that encompasses both memory corruption and micro-architectural side-channel threat models. In this quest, we aim to answer the following questions.

\begin{itemize}
    \item Are any memory corruption mitigations are vulnerable to \ssb attacks? 
    How do we identify and classify the insecure mitigations? % 
    
    \item How does a realistic speculative shield bypass attack exploitation operate?
    Are there common recipes among such \ssb attacks?
    
    \item What new insights can we learn from the analysis? Can these insights be used to guide the design of future memory corruption mitigation mechanisms to be resilient against \ssb  attacks? %\pwd{First sentence of this bullet is redundant}
\end{itemize}

To answer the above questions, we first systematize a taxonomy 
which allows one to reason about the security of memory corruption mitigations against \ssb attacks.
Through this process, we identify two classes of defenses that are likely vulnerable to \ssb attacks, namely ones that utilize tamperable metadata or randomize the address layout. We find that 10 mitigations fall in these two classes of defenses.

Next, we develop a graph-based model to systematically analyze the 10 likely vulnerable defenses and to reason about possible countermeasures. We call our graphs ``\graph{s}''  (\shortgraph{s} for short). \shortgraph{s} help us precisely visualize the information flow between the security checks imposed by the memory corruption defenses and observable microarchitectural events, identifying
sources of microarchitecural side-channel leakage.

To further support our analysis results, we demonstrate the attack vectors through three proof-of-concept attacks, breaking Stack Smashing Protection~\cite{stackguard_canaries}, Always On Heap Memory Safety (AOS)~\cite{aos}, and Cryptographic Capability Computing (C3)~\cite{c3}.

\paragraph{Contributions} 
In summary, we make the following contributions:
\begin{itemize}
    \item A taxonomy which allows one to reason about the security of memory corruption defenses against \ssb attacks
    \item 
    A graph-based model to analyze and reason about side-channel vulnerabilities in memory corruption mitigations.
    %\item A systematic analysis of 20 defense proposals, among which 10 are vulnerable to either one or both of the two attack vectors. 
    \item Three proof-of-concept demonstrations of synergistic attacks.
\end{itemize}



\weon{======================OLD====================}

\asplosdel{Once ASLR is broken, the attackers are free to exploit memory corruption vulnerabilities that were protected by ASLR to perform memory corruption exploits such as control-flow hijacking\hbox{~\cite{jop, rop2012, bittau2014hacking}}.}
%\mengjia{The last sentence is unneccessary. Also add PACMAN...}
%After breaking ASLR, the attacker learns the address of ROP/JOP gadgets and can then exploit a memory corruption vulnerability to construct a code-reuse attack~\cite{code-reuse-attack}.
%\mengjia{we did not make ourselves clear enough. People may think the attack stop here... The importance is that after ASLR is broken, code reuse-attack can work..\\
%After ASLR is broken, the address of gadgets are know, and a code reuse attack can then be conducted....}
%For example, multiple work~\cite{speculativeprobing, hund13, gras17} has demonstrated breaking Address Space Layout Randomization (ASLR)~\cite{pax_aslr, usenix_aslr}, which is intended to protect software vulnerabilities, using cache-based side channels, which exploit hardware vulnerabilities.
%We call an attack \emph{a synergistic attack} if it exploits compound effects of more than one types of vulnerabilities.


%We call an attack \emph{a synergistic attack} if it exploits the compound effects that arise at the convergence of two or more types of vulnerabilities residing in different layers of the system stack.
We call an attack a \emph{synergistic attack} if it exploits the compound effects of vulnerabilities residing in multiple layers of the system stack.
Importantly, in contrast to simply targeting different vulnerabilities, synergistic attacks leverage the diverse caliber of the different attack primitives to assist and empower each other, resulting in substantially more devastating outcomes.\mengjia{come up with a better term that is more specific to what we are doing..}


It is critically important to study synergistic attacks.\mengjia{change this paragraph accordingly when we have a better term, because in this case, we can be more specific with what layers are are talking about.}
\weon{if we start the motivation as ssb, it would make more sense to delete this paragraph entirely. the next paragraph defines ssb.i can discuss more in person.}
\pwd{I agree that defining what the `system stack' is is quite important. It's not clear if you're just narrowly defining this synergistic term to denote attacks across the HW/SW boundary, or across finer boundaries (e.g. HW/Hypervisor/OS)}
\weon{i think i can fix up this section. todo.}

%pose significant security implications.
%On one hand, the ASLR attack examples demonstrated that microarchitectural attacks can help remove the critical barriers for various memory corruption attacks, including the prominent ROP~\cite{rop} and JOP attacks~\cite{xx}.
%On one hand, the ASLR break examples have demonstrated that  micro-architectural attacks can universally remove the significant barriers suppressing memory corruption attacks.
%can help remove the critical barriers for various memory corruption attacks, including the prominent ROP~\cite{rop} and JOP attacks~\cite{xx}.
%\mengjia{I feel the discussion below is a bit verbose and repetitive... we already say they are compound and devastating in the last paragraph.
%You are providing details that might not fit in intro.
%I am thinking maybe we can just talk about these attacks are difficult to mitigate and easy to miss...}
%\weon{Removed the ASLR part. How's now?}
%On one hand, synergistic attacks have demonstrated that ASLR can be broken (1) without any information leakage in software and (2) on anomaly-susceptible programs without causing any architectural anomalies; a feat that is not possible in traditional attacks.
%As synergistic attacks out-perform each of the composed attack strategies, they violate both confidentiality and integrity of the system in ways that were not traditionally possible.
On one hand, synergistic attacks out-perform each self-composed attack strategies,  violating both confidentiality and integrity of the system in ways that were not traditionally possible.
On the other hand, synergistic attacks are easy to miss and difficult to mitigate.
%The main reason is that researchers commonly explore defense mechanisms for each threat model separately.
%To understand synergistic attacks already require researchers to have expertise that span across multiple layers of the system.
Modern systems have a large and complex attack surface.
To handle such non-trivial complexity, security researchers today often partition the problem space into a number of disjoint threat models, exploring each threat model separately. 
To mitigate against synergistic attacks, researchers must first acquire domain expertise that spans across multiple layers of the system stack.

\paragraph{This Paper}
We strive to provide the \emph{first} systematic analysis of one such synergistic threat model; a threat model that encompasses both memory corruption and micro-architectural side-channel threat models.

Specifically, we study \textit{speculative shield bypass} attacks which leverage microarchitectural side channels to leak some secret that is critical to the security of a memory corruption mitigation.
Once a speculative shield bypass attack acquires the secret knowledge necessary to bypass the mitigation mechanisms, it conducts a memory corruption exploit, such as control-flow hijacking.
\pwd{The initial presentation of the term `speculative shield bypass' is confusing in my opinion. At first glance, it sounds like you're talking about an existing `speculative shield' which you're bypassing. It gets clearer as the text progresses, but it would be useful to clarify here what the `speculative' part of ssb actually refers to early on (which you don't do in these sentences)}
\begin{comment}
\asplosdel{
Specifically, our synergistic attacks leverage microarchitectural side channels to leak some secret that is critical to the security of a memory corruption mitigation. %and then use the \pwd{...}
Once our synergistic attacks acquire the secret knowledge necessary to bypass the mitigation mechanisms, we conduct a memory corruption exploit, such as control-flow hijacking.~\footnote{Our synergistic attack is different from speculative control-flow hijacking. More details are in \cref{sec:related}.}}
%\mengjia{very important sentence, need to polish more..}
%\mengjia{talk about the workflow... otherwise... not too clear... otherwise, people might think that we just use speculative execution to bypass bound-check to leak info....}
%We want to answer the following questions.
%In this quest, 
\end{comment}

We aim to answer the following questions.
%\begin{itemize}
%    \item Given the vast number of memory corruption mitigations, which of them are vulnerable to synergistic attacks assisted with microarchitectural side channels? How to classify vulnerable mitigations?
%    \item How does a practical synergistic attack work to bypass a memory corruption mitigation? Does there exist common receipts for such attacks?
%    \item What new insights can we learn from the analysis? Can we use these insights to guide the design of future memory corruption mitigation mechanisms that will be resistant to these synergistic attacks?
%\end{itemize}
\begin{itemize}
    \item %Given the trend of dividing the attack surface into disjoint threat models for defense proposals, are any memory corruption mitigations vulnerable to synergistic attacks? 
    Are any memory corruption mitigations vulnerable to \ssb attacks? 
    %exploiting a combination of memory corruption and side-channel vulnerabilities?
    How do we identify and classify the insecure mitigations? % from the vast and diverse mitigation space? \pwd{This point doesn't make much sense - is there a large `secure' mitigation space?}
    %\item How does a practical synergistic attack work to bypass a memory corruption mitigation? 
    
    \item How does a realistic \asplosrev{speculative shield bypass} attack exploitation operate?
    %How does a realistic synergistic attack exploitation against memory corruption vulnerabilities operate?
    Are there common recipes among such \asplosrev{speculative shield bypass} attacks?
   
   % \item How does a practical synergistic attack work to bypass a memory corruption mitigation? Does there exist common receipts for such attacks?
    %\item What new insights can we learn from the analysis? Can we use these insights to guide the design of future memory corruption mitigation mechanisms that will be resistant to these synergistic attacks?
    \item What new insights can we learn from the analysis? Can these insights be used to guide the design of future memory corruption mitigation mechanisms to be resilient against \asplosrev{speculative shield bypass} attacks? %\pwd{First sentence of this bullet is redundant}
\end{itemize}



%To answer these questions, we start by proposing a taxonomy (\cref{sec:taxonomy}) to characterise a broad range of memory corruption mitigations.
%Note that, for the benefit of the computer architecture community, the majority of the mitigations under analysis have an architectural design component.
%To answer these questions, we start by proposing a taxonomy (\cref{sec:taxonomy}) to classify a broad range of memory corruption mitigations, with a focus on hardware-software co-design schemes.
%Note that, for the benefit of the computer architecture community, the majority of the mitigations under analysis have an architectural design component.
%Different from prior survey work~\cite{sokxx?}, which focuses on how these mitigations block different steps in a memory corruption attack, we focus on analyzing the weaknesses of the mitigation itself and try to understand whether the mitigation mechanism is vulnerable to information disclosure attacks.


%The reason that we care about information disclosure attacks is that microarchitectural side channels are notoriously effective in leaking secrets. 
%According to our analysis, if a mitigation mechanism maintains tamperable metadata or relies on address layout management, it is highly likely that the mitigation mechanism is vulnerable to information disclosure attacks.
To answer the above questions, we first systematize a taxonomy of the state-of-the-art memory corruption defenses 
%focusing on 
that focuses on
hardware-software co-design solutions.
%Using our taxonomy, memory corruption defenses are accurately classified into unambiguous categories.
Based on this taxonomy, we systematically evaluate 20 defenses with a focus on possible weaknesses that can be exploited to either penetrate or bypass the respective defenses.
\mengjia{need to fix the description on taxonomy. 1. our taxonomy is focusing on one specific aspect of memory corruption mitigations; 2. provide the takeaways from our taxonomy: that is mitigations that are using tamperable metadata or relies on address layout randomization are potentially vulnerable to our attack.}
The extensive nature of our taxonomy allows one to easily identify vulnerable attack surfaces particularly due to information disclosure attacks.
%\mengjia{just to make the sentence short... this sentence spans across 5 lines...}
%leading to the discovery of 10 vulnerable defense schemes 
We discover 10 vulnerable defense schemes 
%\pwd{`defense findings' is awk.}, 
among which 5 are either currently deployed, or soon to-be deployed in products by the industry.

Next, we identify that there exist two attack vectors for leveraging speculative execution in our synergistic attacks to bypass memory corruption mitigations, namely by leaking critical metadata or address layout information.
\mengjia{change it to a model, this model will be able to reason about both attacks and defenses.}
%The first attack vector is a Spectre v1~\cite{spectre} and its variants to directly leak metadata stored in memory.
The first attack vector utilizes a Spectre v1~\cite{spectre} primitive or its variants to directly leak metadata that is stored or encoded in the virtual address space.
%The second attack vector is to use speculative execution to suppress crashes to leak security check outcome.
The second attack vector utilizes speculative execution to suppress crashes (and other anomalies) while leaking the (secret) security-check outcome.
%, granting the adversaries the ability to build ``oracles'' that leverage transient brute-forcing primitives.
%\mengjia{what do you mean by "the oracle can leverage brute-force primitive", isn't it that "the orable helps brute-force"?}
%\weon{it means oracles use brute-force primitives for a purpose. not oracles help brute-force}
%We find the vulnerable mitigations are vulnerable either of the two attack vectors.
We find all the 10 vulnerable defenses that we identified in the taxonomy to be vulnerable to either one or both of the two attack vectors.

To further support our analysis results, we demonstrate the attack vectors through three proof-of-concept attacks, breaking Stack Smashing Protection~\cite{stackguard_canaries}, Always On Heap Memory Safety (AOS)~\cite{aos}, and Cryptographic Capability Computing (C3)~\cite{c3}.


%The first two PoCs leverage our first attack vector, \textit{transient de-reference}, to break stack smashing protection~\cite{stackguard_canaries} and Always On-memory Safety (AOS)~\cite{aos}
%\pwd{Might be worth spelling this one out}.
%The third PoC leverages our second attack vector, \textit{transient crash}, 
%\pwd{italicize these attack names}
%to break the address encryption, then leverages our first attack vector, transient de-reference, to break data encryption, penetrating one of the latest academic proposals called Cryptographic Capability Computing (C3)~\cite{c3}.

%\weon{the next two paragraphs starting here are less furnished. they will be modified once the backend of the paper is more stable}
%\mengjia{can add more things when we finish the corresponding sections}
%To further support our analysis results, we showcase three proof-of-concept attacks as below.
%The first two PoC attacks use Spectre to break stack canary and AoS~\cite{aos}, respectively.
%The third PoC attack uses the second attack vector to break one of the state-of-the-art mechanisms called C3 (Cryptographic Capability Computing)~\cite{c3}.
%We demonstrate our attack of stack canary on real processors and the attacks on AoS and C3 on the gem5 simulator~\cite{gem5}.
%In addition, we provide extensive security analysis of multiple other mitigation mechanisms and point out their vulnerabilities.
%For example, we found that Califorms~\cite{califorms}, as one of the very few mitigations that takes speculative execution attacks into consideration, is still fundamentally vulnerable to our synergistic attacks.

\begin{comment}
\mengjia{I feel the impact part is a bit repetative and does not provide more information....
seems removable...} \pwd{I agree}
\paragraph{Impact}
We envision our analysis to have significant impact to both industry and academia. From an industry perspective, our attack vectors not only break the traditional deployed defenses such as stack smashing protection~\cite{stackguard_canaries} and ASLR~\cite{pax_aslr, usenix_aslr}, but possibly the latest features being deployed such as ARM PA~\cite{armpa} and SPARC ADI~\cite{sparc_adi}, and soon-to-be deployed mitigation features such as ARM MTE~\cite{armmte}. Unless additional mitigation measures are taken, we expect our attack vectors to affect the majority of mobile devices as well as many desktop devices in the upcoming years.

From an academic perspective, we have seen a consistent rate of publications in mitigating memory corruption vulnerabilities throughout the last 20 years~\cite{hardbound, watchdog, watchdoglite, aos, chex86, califorms, rest, morpheus, cheri, no-fat,zero,c3}. Among those studied, we only found 3 to consider side-channels in their threat model, and despite the undertaking, 2 to break against our attack vectors \pwd{re-word, this sentence doesn't make sense -- two of the defenses considering side-channels are faulty?}. 
Our work calls for a re-evaluation of how our community defines threat models when proposing a defense. 
We envision our work will inspire more research, exploring both attacks that exploit and mitigations that defend against synergies that arise between vulnerabilities that span across different layers of the system.
\end{comment}

\paragraph{Contributions} 
In summary, we make the following contributions:
\begin{itemize}
    \item A taxonomy of memory corruption mitigation mechanisms to identify whether they are be vulnerable to synergistic attacks. %\yuheng{Do you mean we start to divide these mitigations into two sets, vulnerable to synergistic or not?}
    %\mengjia{information disclousre attack?}\weon{i think it's better to introduce that in the taxonomy? or no? here just simplify it all into synergistic? Too much?}\mengjia{sounds good}
    \item Two attack vectors that can be leveraged during synergistic attacks to penetrate memory corruption mitigations.
    \item A systematic analysis of 20 defense proposals, among which 10 are vulnerable to either one or both of the two attack vectors. %\yuheng{I feel this is closer to the first bullet. While the current second bullet is kind of detail on how to find they are vulnerable.}
    %\mengjia{seems like the first bullet is not clear enough. We actually only say whether a mechanism is vulnerable to information disclosure in taxonomy. may need to refine...} \yuheng{I got the logic after reading the taxonomy section. taxonomy specify something can be leaked, then attack implement them}
    \item Three proof-of-concept demonstrations of synergistic attacks.

\begin{comment}
    \item We perform the first comprehensive analysis of state-of-the-art memory corruption mitigations against synergistic attacks that target vulnerabilities in both hardware and software, and present a taxonomy of these defense mechanisms. 
    Using this taxonomy, we analyze 20 defense proposals and find 10 to be vulnerable 
    %\pwd{Before you said that they were vulnerable, and now you say they're possibly vulnerable?}.
    \item We identify two attack vectors that can be leveraged during synergistic attacks to penetrate memory corruption mitigations. We perform a detailed analysis of each mitigation against the two attack vectors and find all 10 of the possibly vulnerable schemes to be vulnerable to either one or both of the two attack vectors. \pwd{This is a partial repeat of bullet number 1}
    \item We provide three proof-of-concept attack demonstrations against a currently deployed mitigation, stack smashing protection~\cite{stackguard_canaries}, and two state-of-the-art academic proposals AOS~\cite{aos} and C3~\cite{c3}. 
    %We demonstrate 
    %\pwd{[attacks on]} 
    %attacks on SSP on a real machine, and demonstrate attacks on AOS and C3 using an architectural simulator.
    %\item We provide a thorough discussion on countermeasures and related work.
    %\mengjia{it should be ok to exclude the last item..}
\end{comment}
\end{itemize}




%\mengjia{todo... add contribution bullets; maybe add discussions on what we learn from the analysis.}
%Our analysis sheds lights on how to design future mitigation mechanism .....
%\mengjia{my take is that hiding metadata-> maybe possible; hiding layout-> very unlikely, unless use  full spectre mitigation}


\begin{comment}
\begin{scriptsize}
\begin{verbatim}

# Background

- generally consider different threat models separately, this paper strives to consider synergistic attacks 
- what is memory corruption attacks, we call it software bugs, to distinguish from micro-architectural side channel
- microarchitectural side channel, considered to exist at micro-arch layer
- generally people look at them separately; both attacks are broadly affect ....


# Motivation

- several attempts
- several work has demonstrated speculative execution attacks can bypass ASLR
- a good example

# Goal

- mitigations aim to address each of them, but not both
- we try to answer questions:
1. any of the existing memory corruption mitigations can be bypassed by speculative execution attacks?
2. Which features determine whether they are vulnerable?
3. what are practical attack vectors to mitigate these 
4. we want to learn from the systematic analysis to 1) understand the threats; 2) guide the design of mitigations towards future ....

# Contributions

- provide a taxonomy to identify what ... 
- discuss two prominent attack vectors 
- demonstrate 3 case studies
- our taxonomy and analysis method can apply to future mitigation mechanisms



\end{verbatim}
\end{scriptsize}
\end{comment}

==> sections/mld-attempt-old.tex <==

\begin{minted}[fontsize=\footnotesize,      obeytabs=true,tabsize=4,numbersep=3pt,escapeinside=||]{python}
# baseline is vulnerable to Spectre
mld ld-ld-baseline (addr):
    uarch(ld addr);
    |\colorbox{yellow}{data}| = mem[addr];
    uarch(ld |\colorbox{yellow}{data}|+ptr);

# ASLR can leak metadata (segment offset)
# vulnerable to Spectre only after ASLR is bypassed
mld ld-ld-ASLR (addr):
    if addr in [start+|\colorbox{red}{delta}|, end+|\colorbox{red}{delta}|]:
        uarch(Exception); ret;
    else:
        uarch(ld addr);
    |\colorbox{yellow}{data}| = mem[addr]; #only vulnerable to Spectre after ASLR is bypassed
    if (data+ptr) in [start+|\colorbox{red}{delta}|, end+|\colorbox{red}{delta}|]:
        uarch(Exception); ret;
    else:
        uarch(ld |\colorbox{yellow}{data}|+ptr);

# Califorms can leak metadata (segment offset)
# vulnerable to Spectre
mld ld-ld-Califorms (addr):
    uarch(ld addr);
    if addr in |\colorbox{red}{red\_zones}|:
        data = 0;
    else:
        |\colorbox{yellow}{data}| = mem[addr];
    uarch(ld |\colorbox{yellow}{data}|+ptr);

# ARM PA can leak metadata (correct PAC)
# is not vulnerable to Spectre
mld pac-ld-ld-ARM-PA (addr):
    correct_pac = f(addr, |\colorbox{red}{key}|, salt);
    if addr.pac != correct_pac:
        uarch(Exception); ret;
    else:
        uarch(ld addr);

# ARM PA can NOT leak metadata (correct PAC)
# is vulnerable to Spectre
mld ld-ld-AOS (addr):
    uarch(ld addr); #happen in parallel with bound check
    |\colorbox{yellow}{data}| = mem[addr];
    uarch(ld |\colorbox{yellow}{data}|+ptr);
    # in parallel
    bound1 = |\colorbox{red}{table\_lookup}|(addr.pac);
    if addr not in bound1:
        mark Exception; # no observable outcome
    bound2 = |\colorbox{red}{table\_lookup}|((data+ptr).pac);
    if (data+ptr) not in bound2:
        mark Exception;


# NO-FAT can leak metadata (allocation tag)
# is NOT vulnerable to Spectre
mld secld-secld-NO-FAT (addr):
    if |\colorbox{red}{addr.base.temporal\_tag}| != addr.temporal_tag:
        uarch(Exception); ret;
    else:
        uarch(ld addr);
        |\colorbox{yellow}{data}| = mem[addr];
        if |\colorbox{red}{ptr.temporal\_tag}| != (ptr+data).temporal_tag:
            uarch(Exception); ret;
        else:
            uarch(ld data+ptr);


\end{minted}


==> sections/outline.tex <==
%\section{Outline}
%\vspace{+2ex}

\begin{abstract}
\end{abstract}


\weon{discuss weaknesses of each mitigation in section3 (e.g., REST, ZERO(temporal), Intel CET,...}

\weon{start filling in the easy sections 2, 3, 4, 7}
\weon{Are subcategorization after Metadata Modifiable? Static/Dynamic Randomization relevant?}
\weon{re-discuss page permissions in the tabble}
\weon{add metadata type: Infinite Color Tracking, Finite Color Tracking, hashing of VA, random value}
\weon{static layout management: Canary: padding before return address. endbranch: padding before code regions. security bytes: padding around objects}
\weon{make both versions: static layout management vs static layout randomization. compare the differences.}
\weon{forged PAC == rogue PAC... "forging rogue PAC" }
\weon{SafeSEH, SEHOP}
\weon{Intel IBT, ARM MTI: forge branch target locations with JIT}
\weon{Figures to explain C3 attack steps.}

\begin{scriptsize}
\begin{verbatim}

###1. Intro###
\end{verbatim}



\begin{verbatim}

###2. Background###

OR #2.1A History of Memory Corruption Attacks and Mitigations#
- Buffer Overflows 
- Return to Shellcode
- Page Permissions (NW, NX)
- Return to libc/ROP
- Canary
- Function Pointer Overwrite, Non-adjacent Overwrite, UAF
- ASLR

OR #2.1B Taxonomization of Attacks such as in SoK#
- Taxonomization of Attacks we use later in the paper into SoK style.

OR #2.1C Something in between 2.1A and 2.1B

#2.2. Microarchitectural Side-Channel Attacks# 
- Side Channel Attacks
- Speculative Execution Attacks#
    - Increased attack vector for data-tap
    - Speculative Crash-Resistance
    
###3. Focus: Synergies between Memory Corruption Attacks 
and Microarchitectural Side-Channel Attacks

###3. Threat Model###
- Traditional Memory Corruption Threat Model
  - Formalize like DAWG. Talk specifically about Google NaCl or WebAssembly.
- Side-Channel Threat Model
  - Formalize like DAWG. Talk specifically about Spectre. Meltdown.
- Synergistic Threat Model
  - Formalize above together.
\end{verbatim}

\begin{verbatim}

###4. Formalization of Memory Corruption Mitigation 
Through Synergistic Threat Model### 

- Address Augmentation
    - Metadata Modifiable vs Not Modifiable
        - Infinite Coloring vs Finite Coloring vs Hashing of VA vs Random Number
- Address Layout Randomization
    - Static Randomization vs Dynamic


- Code Integrity and Nonexecutable Data
  - Page Permissions
- - ASLR
  - ASLR
- Return Integrity:
  - Canary, Intel CET (SS)
- Control Flow Integrity:
  - Intel CET (IBT), ARM BTI
- Pointer Integrity
  - Data Flow Integrity: ARM PA
  - Data Integrity: ZERO
- Memory Safety:
  - Explicit Base/Bound/Identifier: 
    - Disjoint: Intel MPX, Hardbound, Watchdog, Watchdoglite, CHEx86
    - Inline: CHERI
  - Implicit: No-FAT, C3
  - Co-joined: ARM MTE, SPARC ADI
  - Tripwire: REST, Califorms
  - Randomization: Morpheus
  - Data Encryption (Data Space Randomization)
      - C3 part2, Morpheus part2
\end{verbatim}

\begin{verbatim}
###5. Leakage Model and Attacks ### 

\end{verbatim}

\begin{verbatim}
###6. PoC. ### 

\end{verbatim}


\end{scriptsize}




==> sections/synergisticattacks-old.tex <==

% \mengjia{this section will be completely rewritten...
% model...
% And in Section 6.2, no need to be comprehensive. say we will an appendix to include the model for every scheme, and the S6.2 wil only have examples. Need to pick examples carefully, maybe use the example in the PoC sections.}



% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/SSB-model2.pdf}
%     \caption{Caption}
%     \label{fig:ssb_model}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/SSB-model-v4.pdf}
    \caption{Modeling speculative execution behaviors of memory corruption mitigations when executing the Spectre gadget. {\textcolor{red}{Red}} texts indicate secrets in the mitigation mechanisms, and {\textcolor{blue}{blue}} texts indicate attacker-controlled variables.}
    \label{fig:ssb_model}
\end{figure*}

\section{Modeling Speculative Shield Bypass Attacks}

% \mengjia{a raw draft...}
We use a graph-based model to systematically analyze \ssb attacks on the 10 vulnerable memory corruption mitigations and potential future mitigations.
The goal is to capture the common characteristics of information leakage on different mitigations and understand how to defend against \ssb attacks.


\subsection{Speculative Information Flow Graph}

Recall that, in a speculative execution attack, the attacker triggers secret-dependent speculative execution in the victim program to result in distinguishable micro-architectural side effects.
Therefore, our graph-based modeling approach focuses on tracking and visualizing secret-dependent information flows, including data-flow and control-flow dependencies at the micro-architectural level.
We call our graph a \graph (SIFG).
Prior work~\cite{ruby's understanding paper, Caroline's checkmake} have also used graph representations to understand speculative execution attacks. We discuss how our modeling different from those prior work in \cref{sec:model:discuss}.

% \mengjia{it is unnecessary to invent completely new modeling method. we find our modeling renaissance... we show the key insights are almost the same, capturing execution ordering between operations, but we note the limitations of the original model only used for reasoning of leaking program data due to applying to different threat model in a discussion subsection.}

% Our graph shares a lot of similarities with the Topological Sort Graph used in \cite{ruby's understanding paper}.
In a \graph, a node represents a micro-architectural operation, which may or may not be observable via micro-architectural side channels.
% The granularity of the operations covered by each node is carefully chosen to capture the relationship that is critical for \ssb attacks without embedding unnecessary details. 
For example, a node could be a memory access operation, whose address can be distinguished via cache-based side channels, or a security check operation, which is introduced by a mitigation mechanism and could take various formats (\cref{sec:taxonomy}).
There exist two types of relationships between a pair of nodes.
First, if there exists a directed path from one node the the other, it means there exists a control-flow or data-flow dependency between the two operations, and the two operations are forced to happen sequentially in hardware.
Second, if there does not exist a directed path between the two nodes, it means there does not exist information flow between them and the two operations can happen in any order.
% Note that, different from traditional information flow graphs~\cite{xxx} that describe behaviors at program level from a software perspective, a \shortgraph describes relationships between micro-architectural operations from a hardware perspective.
% The two operations can not be exploited to leak information, since there does not exist information flow between them.

In \cref{fig:ssb_model}, we show the corresponding \shortgraph for each of the mitigation schemes when executing the Spectre gadget \verb|if (cond) {y = ld x; z = ld y;}|.
We highlight the secrets in each mitigation scheme using red texts, and the attacker-controlled variables using blue texts.
These secrets in the mitigation mechanisms are either some tamperable metadata or the randomized offset.
The attacker-controlled variables include the variable $x$ and any metadata embedded inside it.
%excluding ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi}.
% The attacker can control $x$ by supplying the input via a system call to the kernel or an argument to a program.
% Alternatively, the attacker can control the variable by exploiting memory corruption vulnerabilities, as shown in Speculative Probing~\cite{speculativeprobing} and PACMAN attacks~\cite{pacman}. 
We use these graphs to analyze whether and how the secrets can be leaked via \ssb attacks.

% \mengjia{mention that all prior work looks at how to design different security checks/metadata formatting. We focus on the dependency between security checks/authorization and protected operations ...}

\subsection{Modeling Baseline Micro-architecture}
We start with analyzing the baseline micro-architecture to show that the \graph (\shortgraph) is simple and intuitive enough to help us understand how \ssb attacks work.
We use yellow nodes to represent micro-architectural observable events and mark mis-speculation window using shades.
Here, we assume programs are protected via software-only mitigations, using the stack smashing protection~\cite{stackguard_canaries} as an example. 
The secret in the stack smashing protection is the canary, which is stored in addressable virtual memory.


In \cref{fig:ssb_model}(a), within the speculation window, we have two operations.
The first operation performs a load using an attacker-controlled address $x$ and retrieves a potential secret $y$.
This can happen when the attacker makes the value of $x$ match the address which stores the canary.
Next, the second load operation works as a transmission operation as it can leak the value of $y$ (the canary) via cache side channels.
Once the canary value is leaked, the attacker can use the leaked value to spoof security checks and bypass the protection.
We show a proof-of-concept demonstration of attacking the stack smashing protection on a real machine in \cref{sec:poc1}.


\takeaway{If a mitigation metadata is stored in addressable virtual memory, the metadata can be leaked via Spectre and its variants.}



% \begin{verbatim}
% - show the simplicity and intuitive
% - assuming some form of software-only mitigations, here we use stack canary as an example
% - yellow nodes are micro-architecturall observable .... and we mark the specuation window with shades.
% - the secret in the stack canary is stored in addressable virtual memory
% - the graph shows that the first ld instruction takes an attacker-controlled address, and retrieve the potential secret y. this can happen when attacker supplies an x that matches the location that stores the canary => specifically, a secret access operation
% - next the second load is a transmission instruction that leaks the value of y via side channels
% - in this case, canary can be leaked => a transmission operation
% -  the derived canary to spoof security check and bypass the protection
% - we show a PoC of attacking stack canary in S7.1 on a real machine
% \end{verbatim}





\subsection{Modeling Sequentially Guarded Security Checks}

\begin{verbatim}
- almost all mitigations introduce security checks, we use red node to represent security check operations
- the differences lie in the relationship between the security checks and their protected operations
- one of the common approach is to enforce sequential ordering between ...
- we find a group of mitigations, including ....., can fall into this category as shown in b-e
- using aslr as an example
- when executing spectre
    - before performing the first load, a security check to see whether address x is mapped 
    - if x is not mapped, not within the valid region, the speculation window stalls until 
    the branch resolves and decide whether we should squash or commit later
    - if x is mapped, the load operation can proceed which lead to observable micro-arch side effects
    - the same thing happens for the second load
- we call this case security checks sequentially guard the protected operations
- We can identify secret-dependent information leakage paths
    - the security check node
\end{verbatim}



\subsection{Modeling Califorms}

\subsection{Modeling Parallel Security Checks}


\subsection{Discussion}
\label{sec:model:discuss}


\paragraph{Other Mitigation Mechanisms}
.... not covered ARM MTE and SPARC ADI => only secure if it take AOS's design ...


\paragraph{Comparison to Other Graph-based Representations}


% \begin{footnotesize}
% \begin{verbatim}
% - The goal and challenges:
%     - We know: to leak secret via speculative execution attacks, 
%     we need to have secret-dependent distinguishable micro-architectural events
%     - applying this to memory corruption mitigations, we want to find code patterns/execution patterns that can result in different micro-architectural events corresponding to different secret in the protection mechanism
%     - challenge: mitigation mechanism introduce various types of security checks
%     - We need to come up with a systematic way to understand/analyze them
% - High-level approach:
%     - we use a graph model to describe how security checks interfere with the protected instructions (mostly ld/st/indirect br) under speculation
%     - the arrows in a graph clearly describes the data/control dependency between different operations, and they need to be executed sequentially
%     - if there does not exist a path between two nodes, meaning there exist race conditions that can be exploited by attackers to reorder these operations
%     - Used for attack: we can use the graph to identify secret-dependent information flow to micro-arch events and craft SSB attack strategy to leak secret (metadata, or security check outcome)
%     - Used for defense: add or remove edges to mitigate SSB attacks

% - Detailed case by case study
%     1) baseline: -> vulnerable to spectre, discuss stack canary
%     2) ASLR, ARM PA, C3, NO-FAT: -> add security check, can block spectre, 
%     leak secret-dependent security check outcome by observing whether a load happens
%     3) Califorms -> leak secret (redzone) by distinguishing speculative load addresses
%     4) AOS: do not block Spectre at all, like baseline
%     5) ARM MTE and SPARC ADI: could be either case
    
% - Discussion
%     - our graph model is very similar to Ruby's work
%     - we both capture dependency and race conditions
%     - Different threat model and different conclusions
%         - Ruby's conclusion: the lacking of edges in the graph results in race condition, which can be considered as the root cause of speculation attacks
%         - Our conclusion: we consistently observe that edges between security check and the corresponding protected operations result in secret-dependent information flow
%         and results in information leakage of metadata
%         - Why conclusion different? Threat model is different, in our case, the security check 
%         is not trusted, since attacker can tamper the metadata and we are trying to leak security check outcome
%         But in ruby's case, the security check is always trusted
       
% \end{verbatim}
% \end{footnotesize}


Recall from \cref{sec:threatmodel}, our speculative shield bypass (SSB) attack workflow consists of two steps.
In the first step, an attacker exploits a side-channel vulnerability to gain some secret that is critical to a memory corruption defense, such as metadata or address layout information.
In the second step, the attacker leverages the leaked secret to bypass the respective memory corruption defense and performs some memory corruption exploit such as control-flow hijacking.
In this section, we focus on step 1 of the synergistic attack workflow and study how to leak secrets of different mitigation mechanisms, since the step 2 follows the standard memory corruption attacks.\mengjia{TODO: rewrite this paragraph.}






After performing a thorough analysis of the 10 mitigation examples, we identified that there exist two main attack vectors to leak critical metadata or address layout information via speculative execution attacks:
1) using a Spectre v1 primitive or its variations to leak the secret that is stored or encoded in virtual memory, 
or 2) leaking security-check results by observing speculative exceptions. 
%After performing a thorough analysis of the 10 mitigation examples, we identify that there exist two main attack strategies, 1) directly using Spectre v1 and its variations to leak the secret that is stored or encoded in virtual memory, or 2) leaking security check results via observing speculative exceptions. 
We describe the two attack vectors and compare their differences in applicable conditions and attack bandwidth.
%We then discuss how each of the 10 vulnerable mitigations can be bypassed using the two strategies, summarized in \cref{tab:attack-strategy}.

%\mengjia{TODO: is transient crash the good name for the second attack strategy? can we think of %something better?}
%\weon{I'm okay with transient crash -- pretty easy to understand what the name implies -- the crash is rolled back, but leaves micro-architectural trace. maybe there is something better tho... the only one on my mind is something right now is sth more general like -- transient anomaly (but i think transient crash is better than that...}

\paragraph{Attack vector 1: transient de-reference}
%\mengjia{I am trying to introduce the two attack strategies and give them names: transient de-reference, and transient crash. TODO: polish...}
The first attack vector utilizes a Spectre v1 primitive or its other variations to directly leak the secret inside the defense scheme.
%Spectre can be used to construct a universal read gadget, meaning that it can be used to leak every byte in the victim's virtual address space.
This attack vector works only if the defense scheme stores or encodes the secret in virtual memory.
For example, stack smashing protection~\cite{stackguard_canaries} places a (secret) random value (called canary) in the virtual memory, adjacent to the saved return address on the stack.
ASLR~\cite{pax_aslr, usenix_aslr} encodes secret inside the virtual memory by adding a random offset to the code and data segments.
%The first attack vector is to use Spectre v1 and its other variations to directly leak the secret maintained by the mitigation mechanism.
%Spectre can be used to construct a universal read gadget, meaning that it can be used to leak every byte in the victim's virtual address space.
%This attack strategy works only if mitigation mechanisms store or encode secret in virtual memory.
%For example, stack canary~\cite{stackguard_canaries} places a random value (i.e., the canary) adjacent to the saved return address on the stack.
%ASLR~\cite{pax_aslr, usenix_aslr} encodes secret in the virtual memory by adding a random offset to the code and data segments.

\paragraph{Attack vector 2: transient crash}
In the case that the secret does not exist in the virtual memory and cannot be leaked via Spectre (i.e., transient de-reference), an attacker can try to leak the secret \emph{indirectly} using the second attack vector by detecting a \emph{transient crash}.
%The second attack strategy works even if the secret does not exist in the virtual memory.
As the secret is used to perform security checks, the security check outcome, if leaked, can be used to infer the secret.
%As in these mitigation mechanisms, secret is used to perform security checks and the security check outcome, if leaked, can be used to infer the secret.

%If the adversary can control the input to the security check and speculatively leak the security check outcome, the adversary will be able to brute-force the input and eventually leak the secret. 
%, such as checking whether the re-computed PAC value matches the actual PAC value stored in the high bits in ARM PA (\cref{sec:pacman}).
To understand how the secret can be leaked, consider the example attack gadget below.
\begin{minted}[frame=single,obeytabs=true,tabsize=4,numbersep=3pt,linenos,escapeinside=||,fontsize=\small]{c}
 if (cond) { // a mis-predicted branch
    x = security_check(guess);
    y = array[x];  // transmit instruction
 }
\end{minted}

The attack gadget above starts with a branch (on line 1) which may mis-predict and create a speculative execution window.
During this window, the attacker can trigger a security check (line 2) on an attacker-controlled input (the variable \texttt{guess}).
If the guess is correct and the security check passes, an appropriate output value $x$ will be generated.
Otherwise, an exception will be generated which would crash the program, if the instruction were to commit.
However, since the security check is performed under the shadow of a mis-predicted branch, the instruction will be squashed and the corresponding exception will be suppressed.
We call such an exception a \emph{speculative exception}.

%The attack gadget above starts with a branch (on line 1) which mis-predicts and creates a speculative execution window.
%The attacker then triggers a security check using an attacker-controlled input, i.e., the variable \texttt{guess}.
%If the guess is correct and the security check is passed, an appropriate output value $x$ will be generated.
%Otherwise, an exception will be generated and could have crashed the program if the instruction commits.
%However, since the security check is performed under the shadow of a mis-predicted branch, the instruction will be squashed and the corresponding exception will be suppressed.

Following the security check instruction, the gadget contains a transmit instruction (line 3) that transmits the security check outcome via microarchitectural side channels.
Specifically, the transmit instruction performs a data-dependent operation using the security check outcome.
This transmit instruction can be any instruction that causes observable side-effects in the system, and the most common is a memory instruction.
Note that, the attacker only cares about whether the transmit operation itself has \emph{happened} or not, and does not care about the actual value in $x$.
With the ability to discern the security check outcome, the attacker can brute-force the variable \texttt{guess} until it passes the security check.
%This transmit instruction can be any instructions that can cause observable side effects in the system, and the most commonly used one is memory access instruction.
%Note that, the attacker only cares about whether the transmit operation itself has \emph{happened} or not, and does not need to know the actual value in $x$.
%Being able to discern the security check outcome, the attacker can brute-force the variable \texttt{guess} until it can pass the security check.

The security check operation can take on various forms and can be triggered by different types of instructions depending on the mitigation mechanism.
For example, in ASLR~\cite{pax_aslr, usenix_aslr},%, it could be triggered by a load instruction or a function call instruction which 
the security check is performed during address translation by the MMU for memory access instructions. %loads and function calls.
%\mengjia{I want to say what security check is done here... note that  load/function call can also be used as a transmit instruciton.}
%Usually the MMU checks whether the given address points to a mapped region or not and whether the permission of the mapped page is proper.
%Upon accessing an unmapped page or detecting an illegal page permission, a page fault will be generated.
Speculative Probing~\cite{speculativeprobing} first leveraged this approach to bypass ASLR.
In our analysis, we found several additional defenses to be vulnerable to this attack vector, including ARM PA~\cite{armpa}, No-FAT~\cite{no-fat} (regarding temporal safety) and C3~\cite{c3}. 
%are also vulnerable to this attack strategy.

%Note that, the security check operation can take on various forms and can be triggered by different types of instructions depending on the mitigation mechanism.
%For example, in ASLR~\cite{pax_aslr, usenix_aslr}, it could be triggered by a load instruction or a function call instruction that takes on an attacker-controlled address.
%Usually the MMU checks whether the given address points to a mapped region or not and whether the permission of the mapped page is proper.
%Upon accessing an unmapped page or detecting an illegal page permission, a page fault will be generated.
%Speculative Probing~\cite{speculativeprobing} leveraged this approach to successfully bypass ASLR.
%We find several other mitigation mechanisms, including ARM PA~\cite{armpa}, NO-FAT (the temporal safety part)~\cite{no-fat}, and C3~\cite{c3} are also vulnerable to this attack strategy.


\begin{table*}[t]
\footnotesize
    \begin{center}
    %\mengjia{1. secret stored in memory -> secret stored/encoded in memory, in this way, we should also check ASLR, Morpheus, or maybe something more. These stuff can be leaked via secondary software vulnerabilities;\\
    %2. ASLR can be leak via both transient de-refernece and crash, same thing applies to morphedus. Note that Speculative Probing have multiple probe methods.}
    %\small
    \begin{tabular}{|c|c||c|cc||cc|}\hline
    & &  \multicolumn{3}{c||}{\textbf{What to Leak}}  & \multicolumn{2}{c|}{\textbf{How to Leak}}  \\\cline{3-7}
         &\textbf{Scheme} &  \multirow{2}{*}{secret}  & in virtual &  speculative & Transient    & Transient  \\ 
    &       &          &  memory?   &  exception?   & De-reference & Crash \\ \hline\hline
    \multirow{3}{*}{Group A} & Stack  Canary~\cite{stackguard_canaries} & canary & \checkmark & \checkmark &  \checkmark & \checkmark \\%\cline{2-7}
    % & Canary~\cite{stackguard_canaries} &   &   & &   &  \\\hline
    %Protection & & & & \\\hline
     & ASLR \cite{pax_aslr, usenix_aslr} & segment offset & \checkmark &\checkmark & \checkmark & \checkmark \\%\cline{2-7}
    %&  &  & & & \\\hline
     & Morpheus \cite{morpheus} & segment offset  & \checkmark & \checkmark & \checkmark & \checkmark \\\hline%\hline
    %& \cite{morpheus}& Offset & & & \\\hline
    \multirow{2}{*}{Group B} & AOS~\cite{aos} & PAC\textsuperscript{$*$} & \checkmark & x & \checkmark & x \\%\cline{2-7}
     & Califorms \cite{califorms} & address of security bytes & \checkmark & x & \checkmark & x \\\hline%\hline
    %& \cite{califorms}& bits~\footnote{califorms-sentinel in L2 and beyond, and califorms-bitvecotr in L1} & & & \\\hline
    \multirow{3}{*}{Group C} & ARM PA~\cite{armpa} & PAC\textsuperscript{$*$} & x  & \checkmark & x & \checkmark\\%\cline{2-7}
     & No-FAT~\cite{no-fat} & allocation tag\textsuperscript{$\dagger$} & x  & \checkmark & x & \checkmark \\%\cline{2-7}
    %&PA~\cite{armpa} &  &  &  & \\\hline
     & C3~\cite{c3} & cryptographic address  & x  & \checkmark & x & \checkmark\\\hline%\hline
    %& & phic Address & & & \\\hline
    \multirow{2}{*}{Group D} & ARM MTE~\cite{armmte} & memory  tag & x & ? & x & ? \\%\cline{2-7}
    % &  &    &  &  &  \\\hline
     & SPARC ADI~\cite{sparc_adi} & memory tag & x & ? & x & ? \\\hline
    % &  &  Tag &  &  &  \\\hline
    %&\cite{no-fat} &    &  &  &  \\\hline
    \end{tabular}
    \end{center}
    \vspace{-5pt}
    {\small \textsuperscript{$*$}ARM PA and AOS use PACs differently. AOS generates a PAC for every heap pointer at allocation time which then persists until the allocation is freed; hence a heap pointer is stored with its PAC in virtual memory.
    ARM PA generates PACs for pointers at the beginning of critical sections of the program, but ROP/JOP gadget addresses generally do not include PACs because they were not initially signed; thus the secret PAC is not stored in memory.
    \textsuperscript{$\dagger$}No-FAT keeps two different types of metadata for spatial safety and temporal safety, respectively; the allocation tag is used for temporal safety only.}
    \caption{Analysis of two attack vectors on 10 mitigation mechanisms. }

    \label{tab:attack-strategy}
\end{table*}



\paragraph{Comparison}
Comparing the two attack vectors, we can see that they work in very different conditions.
%Comparing the two attack strategies, we can see that they work with different conditions.
The transient de-reference attack strategy requires the secret to be stored or encoded in the virtual memory.
The transient crash attack strategy requires the security check failures to generate speculative exceptions.


In addition, the two attacks have very different attack bandwidth.
%Moreover, the two attacks have very different attack bandwidth.
Transient de-references directly leak the secret value, meaning multiple bits per leak.
%Transient de-reference (i.e. Spectre) can directly leak the secret value, meaning multiple bits for each leakage.
In comparison, the transient crashes leak a boolean value of the security check outcome, i.e. whether the check fails or not.
%However, the transient crash attack strategy most time can only leak a boolean value of the security check outcome, either the check fails or not.
Thus, if secret is the n-bits, one must brute-force upto $2^n$ iterations.
%the bandwidth of the transient crash vector is 1 bit per transient crash invocation.
%\pwd{I don't like this bitwise taxonomy -- say if you have to guess a 16 bit random number, it will take more than 16 transient crashes, no?}
%\mengjia{yes, yes, but how generally do we say this?}
%\weon{can we just remove the last sentence? How do you feel?}
%Therefore, the bandwidth of the second strategy is 1 bit per time, much lower than the first strategy.

\paragraph{Entropy} 
%As transient crash primitives empower an attacker with the ability to build oracles that can reverse engineer the secret, the entropy of these defense mechanisms are important.
As the transient crash primitive requires the attacker to brute-force the secret, the entropy of these defense mechanisms largely determines the feasibility of such attacks.
Unfortunately, as AOS, ARM PA, No-FAT, ARM MTE, and SPARC ADI leverage unused upper bits of a pointer, the entropy of these mechanisms vary between 4 to 17 bits, which is not enough to defend against brute-force attacks.
%Califorms leverages the transient de-reference primitive to build an oracle, but the entropy of redzone limited to 7 adjacent address locations.
In Califorms,  the entropy of the size for each redzone is only 8 (i.e. 3 bits).
The entropy of ASLR on a 64-bit system is between 19 bits (Windows) to 28 bits (Linux heap)~\cite{oregon-slides}.


\subsection{Vulnerabilities to Synergistic Attacks}
\label{sec:vulnerabilityanalysis}

%\mengjia{need a better section title}

%\mengjia{it is a very raw draft.
%What I actually want for each group is to explain the following things in order if possible:\\
%say this group is vulnerable to X or Y or both\\
%1. explain the mechanism if needed;\\
%2. point out the secret in the scheme -> column 3;\\
%3. explain whether secret in virtual memory or not -> column 4;\\
%4. explain whether security check failure causes speculative exception or not -> column 5;\\
%5. explain how to attack...}
%\weon{i think it's pretty hard to skip explaining the mechanism except for the ones discussed elsewhere like ASLR, and pocs...}

We conducted a thorough analysis of the 10 mitigation mechanisms that spanned the two vulnerable categories highlighted in \cref{tab:taxonomy} and found that they can be divided into four groups based on which attack vectors can be utilized against them.
%We perform a thorough analysis of the 10 mitigation mechanisms that span the two vulnerable categories highlighted in \cref{tab:taxonomy} and find that they can be divided into four groups based on which attack strategies work towards them.
We summarize our analysis results in \cref{tab:attack-strategy}, including 
1) what secret value needs to be leaked to bypass the security mechanism (column 3), 
2) whether the secret is stored or encoded in virtual memory 
%\pwd{minor nitpick, but would it be more accurate to say that they're stored in virtual memory \textit{addresses}?}
%\mengjia{my older version is stored or encoded in virtual memory...}
(column 4), and 
3) whether a security check in the mitigation mechanism can cause a speculative exception (column 5).
%We summarize our analysis results in \cref{tab:attack-strategy}, including 1) what secret value needs to be leaked to bypass the security mechanism (column 4), 2) whether the secret is stored in virtual memory (column 5), and 3) whether a security check in the mitigation mechanism can cause a speculative exception or not (column 6).
%\mengjia{I added this sentence, so that later we do not need to point the column numbers any more....} 
We demonstrate proof-of-concept attacks targeting 3 of these mitigation mechanisms from different groups in \cref{sec:poc}.
%We selectively demonstrated PoC attacks targeting 3 of these mitigation mechanisms from different groups in \cref{sec:poc}.

\paragraph{Group A: Stack canary~\cite{stackguard_canaries}, ASLR~\cite{pax_aslr, usenix_aslr}, Morpheus~\cite{morpheus}}
The mitigation mechanisms in group A are vulnerable to both the transient de-reference and transient crash attack vectors.
As previously discussed, both stack canary and ASLR stores or encodes the secret in memory, and thus the secret can be leaked directly using a Spectre v1 primitive.
In addition, stack canary performs an integrity check of the canary value before executing a \texttt{return} instruction (in software) and ASLR performs a security check of each memory access inside the MMU.
%As discussed before, both stack canary and ASLR stores or encodes the secret in memory, and thus can be leaked via Spectre directly.
%In addition, stack canary performs an integrity check of the canary value before executing a \texttt{return} instruction.
%This integrity check operation is implemented in software and can trigger speculative exception when failed.
%ASLR relies on MMU to perform security checks on every memory access.
These operations will generate transient exceptions when the checks fail, while transmitting the check outcomes via micro-architectural side-channels.

%\weon{we need to be careful with Morpheus. They do take traditional side channels and brute-forcing crash resistant programs into their epoch size.}
%\mengjia{how do they consider side channel?}
Morpheus~\cite{morpheus} is a dynamic ASLR scheme, which periodically re-randomizes segment offsets. 
%Morpheus~\cite{morpheus} is a dynamic ASLR mechanism, which periodically re-randomizes address offsets to make the system more resilient to information leakage attacks.
In \cite{morpheus}, the re-randomization epoch size is set to 50ms.
When only memory corruption attacks are considered, this epoch size is reasonable since it is extremely challenging to leak the randomized offset by brute-forcing crash-resistant programs. 
%This epoch size is reasonable since it is extremely challenging to leak the randomized offset by exploiting a secondary software vulnerability within such a short epoch.
However, we suspect that Morpheus may have overlooked the fact that detecting transient crashes via micro-architectural side channels are much faster and each iteration of the attack and may only take a few hundred nanoseconds. 
%\mengjia{why still brute-force... why not directly leak like ASLR?}
If synergistic attacks are considered, Morpheus may need to largely reduce the re-randomization epoch size, which may significantly increase its performance overhead.
%If synergistic attacks are considered, Morpheus will need to largely reduce the re-randomization epoch size, which can potentially significantly increase its performance overhead.


\paragraph{Group B: AOS~\cite{aos} and Califorms~\cite{califorms}}
The mitigation mechanisms in group B are only vulnerable to the transient de-reference attack vector.
%The group B mitigation mechanisms are only vulnerable to the transient de-refernece attack strategy.
We defer the discussion on AOS to \cref{sec:poc2} with our proof-of-concept demonstration, and focus our analysis on Califorms here.
%We defer the discussion on AOS to \cref{sec:poc2} with our proof-of-concept demonstration, and focus on analyzing why Califorms is vulnerable to Spectre for now.



Califorms builds upon the idea of memory blacklisting by adding a random number (between 1-7) of security bytes around allocated sub-objects, and marking these bytes as red zones.
If a memory access touches one of these security bytes, Califorms catches the access in hardware and causes an exception leading the program to crash.
%Califorms builds upon the idea of memory blacklisting by adding a random number of security bytes around allocated data structures and marking these bytes as red zones.
An example code snippet is shown below where \texttt{buf} and \texttt{fp} are protected by the security bytes around them.
\begin{minted}[frame=single,obeytabs=true,tabsize=4,numbersep=3pt,linenos,escapeinside=||,highlightlines={3,5,7},highlightcolor=pink,fontsize=\small]{c}
struct A {
    // security bytes with a random size
    char security_bytes[3]; // red zone
    char buf[64];
    char security_bytes[7];
    void (*fp)();
    char security_bytes[2];
}
\end{minted}

Since the size of the red zone is random, Califorms works as an address layout randomization scheme that operates at a fine-grained byte granularity.
The secret maintained by Califorms is the addresses of the security bytes, which add accumulative random offsets to user-allocated data structures.
Therefore, if the attacker is able to leak the address of the added security bytes, Califorms can be bypassed using a non-adjacent buffer overflow (\cref{sec:bac_memattack}).
%Therefore, Califorms can be bypassed if the attacker is able to leak the addresses and sizes of the added security bytes.
%We note the secret of Caliform is encoded in the virtual address space, as listed in \cref{tab:attack-strategy}.


Proposed after the initial finding of Spectre attacks~\cite{spectre, horn2018speculative, meltdown}, Califorms takes Spectre into its threat model, returning $0$ for speculative loads to security bytes. %leveraging hardware support.
%\mengjia{commonly you put important information at the later part of a sentence. Josep said reading a sentence is like to take a breath, you have a deeper memory of what comes later. So I suggest not using "leveraging hardware support" to end this sentence, since this is not important information.}
However, we found that such a scheme leads to new unsought vulnerabilities against speculative execution attacks.
%Califorms leverages hardware support to perform the security check.
%Specifically, accessing the red zones non-speculatively will result in crashes. 
%In order to avoid leaking the content inside the security bytes, Califorms was designed that any speculative accesses to the red zones will return value $0$~\cite{califorms} and will not generate speculative exception.
%However, we find that such a scheme is far from sufficient to be secure against speculative execution attacks.
The reason is that the secret is the \emph{addresses} of the security bytes, not the \emph{content}.
Thus, an attacker can use a Spectre v1 primitive to speculatively scan the victim's virtual memory and distinguish addresses containing security bytes from valid data, by distinguishing addresses which speculatively return zero.
%The attacker can use Spectre to speculatively scan the victim's virtual memory and distinguish security bytes from valid data bytes by checking whether the speculative accesses return zero or non-zero values.
For example, as long as the the variables \texttt{buf} and \texttt{fp} in the above code snippet contain non-zero values, the addresses of the security bytes can be fully recovered by an attacker.
%\mengjia{shall we talk about false positives? seems unnecessary.}
%\weon{i agree.}




\paragraph{Group C: ARM PA~\cite{armpa}, No-FAT~\cite{no-fat}, and C3~\cite{c3}}
The mitigation mechanisms in group C are only vulnerable to the transient crash attack vector.
We defer the discussion on C3 to \cref{sec:poc3} with our proof-of-concept demonstration, and focus our analysis on ARM PA~\cite{armpa} and No-FAT~\cite{no-fat} here.
%We provide a discussion on ARM PA~\cite{armpa} and No-FAT (temporal safety)~\cite{no-fat} at this moment and defer the discussion on C3 in \cref{sec:poc3} with our PoC demonstration.


%\mengjia{Not too happy about this paragraph .... need some work. Or we should keep it short.. Really hope that we can directly cite PACMAN...}
%\weon{Took an iteration. I think its okay for now... Pretty condensed as it is...}
ARM Pointer Authentication (ARM PA) protects the integrity of pointers.
It introduces two sets of instructions performing the following two distinct set of operations.
%ARM Pointer Authentication (ARM PA) blocks control-flow hijacking attacks by verifying the integrity of pointers. 
%It introduces two sets of instructions performing the following two operations respectively.
\texttt{pacia} instruction and its variants compute a cryptographic hash of a given pointer with a secret key and its context.
%First, the \texttt{pacia} instruction and its variants.
%\This instruction and its variants compute a cryptographic hash of a given pointer with a secret key and its context salt.
The hash is called Pointer Authentication Code (PAC for short), and is stored in the unused bits with the pointer.
\texttt{autia} instruction and its variants check whether a pointer has been tampered with by re-computing the PAC for the pointer and comparing the re-computed PAC against the PAC stored in the upper bits of the pointer.
%Second, the \texttt{autia} instruction and its variants. 
%This instruction checks whether a pointer has been tampered with or not by re-computing the PAC for the pointer and comparing the re-computed value against the PAC values stored in the pointer.
If the two PAC values match, the processor strips the PAC value from the pointer and generates a valid pointer, which can be used normally later.
If the PAC values do not match, it means the pointer has been illegally tampered with.
In this case, the instruction will leave garbled bits inside PAC bits and output an invalid pointer, which will trigger exception when used.
%The instruction will leave garbled bits as PAC bits and output an invalid pointer, which when used, will trigger exception.
%The secret in ARM PA is the correct PAC value of an attacker-controlled pointer, which should point to some payload code or ROP/JOP gadgets.
%Since the victim program itself does not generate PAC values for payload addresses, we consider the secret does not exist in the virtual memory (column 5).


%Considering ARM PA has the above features, we believe our transient crash attack can be used to leak the verification outcome speculatively without causing system crashes.
According to our analysis, ARM PA can be bypassed by transient crash attacks.
The code snippet below shows an example of a function epilogue when ARM PA is used.
%The code snippet below shows the function epilogue when using ARM PA.
\texttt{x30} is the linker register in ARM (line 1) and is used later by the \texttt{ret} instruction (line 4).
%\texttt{x30} is the linker register in ARM and will be used by the \texttt{ret} instruction (line 4).
The \texttt{autia} instruction (line 3) checks the PAC value in \texttt{x30} using the stack pointer \texttt{sp} as the context.
This instruction serves as the security check operation in our transient crash attack primitive.

\begin{minted}[frame=single,obeytabs=true,tabsize=4,numbersep=3pt,linenos,escapeinside=||,fontsize=\small]{as}
ld  x30, sp   // x30 is the linker register
add sp, sp, 0x8
autia x30, sp // security check
ret           // transmit instruction
\end{minted}

If the security check is passed, the following \texttt{ret} instruction will be executed which can be detected using microarchitectural side-channel attacks.
%If the security check is passed, the followed \texttt{ret} instruction will be executed and detected by attackers via microarchitectural side-channel attacks.
If the security check fails, the \texttt{ret} instruction will trigger a speculative exception and an attacker will not observe its corresponding side effects.
Therefore, an attacker can distinguish the security check outcome.
With this primitive in hand, an attacker can speculatively brute-force different PAC values under a branch mis-prediction window, until they find the PAC that passes the authentication.
%With this primitive in hand, the attackers can brute-force different PAC values until they find the correct one.
%ARM PA is widely used in Apple silicon. A PoC attack will require extensive efforts in reverse engineering of this unknown microarchitecture.
%In this paper, we focus on providing a systematic security analysis of a broad mitigation mechanisms and consider a PoC attack targeting ARM PA on real processors as future work.
%\mengjia{a bit verbose..., need to discuss how to better structure this section.}
%We do demonstrate a PoC attack of using transient crash on C3 in \cref{sec:poc3}.

%\mengjia{TODO: we need to explain No-FAT....
%No-FAT stores the temporal tag with the base address and if the tag does not match, it will not use the data....}

The metadata in No-FAT~\cite{no-fat} can be leaked similarly.
To achieve temporal safety, No-FAT generates a random number as a temporal tag and stores the tag with the pointer.
In parallel, the tag is also stored with the allocation address and which is generated by the compiler and maintained by the hardware.
%Besides, the tag is also stored with the allocation address and tracked by compilers.
For example, in the code below, a \texttt{secure\_load} (a new type of load instruction introduced by No-FAT) will obtain (1) the pointer's tag from the upper bits of the variable \texttt{addr} and (2) the tag to be compared against, by inferring the tag location from the variable \texttt{base}. 
%\mengjia{confusing.... the compiler generates the base.. the hardware will track the tag for base... no?}
Next, they will transparently be checked whether they match.
%For example, in the code below, a \texttt{secure\_load} in No-FAT will obtain the tag from the \texttt{addr} and the tag associated with the \texttt{base} address and check whether they match or not.
%The scheme replies on the confidentiality of the temporal tag to be secure.


\begin{minted}[frame=single,obeytabs=true,tabsize=4,numbersep=3pt,linenos,escapeinside=||,fontsize=\small]{as}
if (cond)
  data = secure_load(addr, base) //No-FAT's new inst
\end{minted}

Proposed after the initial finding of Spectre attacks~\cite{spectre, horn2018speculative, meltdown},  No-FAT takes speculative execution into its threat model. 
Specifically, in No-FAT, the hardware detects tag mismatches for \texttt{secure\_load} instructions, before issuing the load to the memory hierarchy, blocking speculative use-after-free accesses. 
However, we found that such a scheme leads to new unsought vulnerabilities against transient crash attacks. In particular, a \texttt{secure\_load} instruction will transmit a signal through micro-architectural side-channels when the tag-check passes, but will trigger a speculatively exception otherwise. Hence, an adversary gains the ability to distinguish the security check outcome.

%No-FAT was designed by taking speculative execution attacks into consideration and was designed to block speculative use-after-free access.
%Specifically, the No-FAT hardware makes the \texttt{secure\_load} instruction immediately detect tag mismatch before issuing the load to the memory hierarchy.
%Therefore, the \texttt{secure\_load} instruction is used both as the the security check instruction and the transmit instruction to leak the check outcome.
%\mengjia{is this paragraph clear?}
%\weon{yes i think so.}



\paragraph{Group D: ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi}}
We consider ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi} in our last group highly likely to be vulnerable to transient crash attacks, but we do not draw conclusions as the micro-architectural details are proprietary and publicly unavailable.
%We consider ARM MTE~\cite{armmte} and SPARC ADI~\cite{sparc_adi} in our last group highly likely to be vulnerable to transient crash attacks, but we cannot conclude since they use proprietary hardware design with microarchitectural details that we do not have access to.

%\mengjia{here...}
%But we do consider that they are highly likely to be vulnerable to 
%\mengjia{need polish}
ARM MTE and SPARK ADI are both memory coloring schemes. Specifically, they maintain a random number tag, which can be denoted as a color, in the pointer and also associate each unit of memory granule with a color.
%Both ARM MTE and SPARK ADI uses a memory coloring scheme.
%They maintain a random number tag, which can be denoted as a color, in the pointer and also associate each unit of memory region with a color.
Upon a pointer de-reference, a security check is performed by comparing whether the color of the pointer matches the color of the referenced memory granule.
%Upon de-referencing a pointer, a security check is performed by comparing whether the color of the pointer matches the color of the referenced memory region.
ARM MTE and SPARC ADI use a 4-bit tag (i.e., 16 colors) for every 16-byte or 64-byte memory granule respectively.
%If the attacker attempts to modify a pointer to point to a different region, the attacker will need to know the color of the target region.
If an attacker attempts to modify a pointer to access a region with a different color, the program will crash.

Since both schemes store the memory tag (the color for each memory granule) in specialized hardware structures, the tag cannot be directly leaked using speculative de-reference attacks.
However, if speculative tag check failures generates transient exceptions similar to ARM PA and No-FAT, these schemes will be vulnerable to transient crash attacks.

%As a result, whether the two mechanisms are vulnerable is completely implementation dependent.
%If a tag comparison failure generates a speculative exception, as how ARM PA and No-FAT does, these two schemes will be vulnerable to transient crash attacks.


\paragraph{Interesting findings}
%Among the ten mitigation mechanisms analyzed in this section, most of them consider speculative execution attacks out of scope.
Among the 10 defense proposals analyzed above, we found most of the proposals to consider side channel attacks as out of scope.
%Only two of them, Califorms~\cite{califorms} and No-FAT~\cite{no-fat}, actually take speculative execution attacks into consideration.
Specifically, we found only two, Califorms~\cite{califorms} and No-FAT~\cite{no-fat}, to consider speculative execution attacks.
%However, we note that neither of the two mechanisms are resistant to our synergistic attacks, that is, the secret that the mitigation mechanism relies on can be leaked via speculative execution attacks.
However, we note that neither of the two mechanisms are resistant to our synergistic attacks, that is, the secret that the defense relies on can still be leaked using speculative execution attacks.
Our detailed analysis plays an important role in helping us to understand why these two mechanisms fail.

%, despite considering speculative execution attacks.
Califorms~\cite{califorms} attempts to hide the content of security bytes from being leaked via speculative execution and makes speculative accesses to these locates to always return $0$.
However, according to our analysis, the secret in Califorms should be the addresses of these security bytes, not the content of the security bytes.
%The attacker can still distinguish security bytes from valid data bytes and thus can recover the randomized offsets.
As an attacker can still distinguish security bytes from valid data, the randomized size of the security bytes can recovered.

%\mengjia{did some tweak. @weon check..}
No-FAT~\cite{no-fat} narrowly considers Spectre v1 and blocks speculative out-of-bound accesses and speculative use-after-free accesses from leaking program data.
However, it does not protect against its metadata from leakage.
As such, the temporal tag, which is used for security check during speculative execution, can be leaked via transient crashes.
%In summary, our analysis highlights that it is non-trivial task to design memory corruption mitigation mechanisms that are resistant to synergistic attacks.
%\mengjia{change it to emphasize the difference between leaking program data and leaking mitigation metadata...}

%\mengjia{synergistic attack? I tried to say speculative execution attacks. But it is very misleading. see No-FAT, which is effective towards Spectre, but cannot protect the secret. Secret is alway vague. So I am struggling here.} \weon{both works. i would argue that attacking memory corruption mitigation using side-channel attack is by definition synergistic, b/c once you break a memory corruption defense, your next goal would naturally be to exploit a memory corruption bug (now that there is no defense -- also -- why would you break the defense, otherwise?) I think you're pointing out No-FAT is kind of also spectre defense, so its tricky, but i would argue our example is breaking temporal safety defense, so the goal of the attacker must be to exploit a temporal vulnerability (even though we don't explicitly say it yet). regarding secret -- in our case the temporal tag is the secret, which we leak via transient crashes. i think you're pointing out that secret is generally dependent on the context, so you're worried the reviews will have trouble understanding?}
%\mengjia{I think as long as we talk about the two steps of our synergistic attacks in the begining of S3.3 or S3.4, we are good. I was feeling uncomfortable because we did not define synergistic attack in our paper explicitly/precisely about the two steps.}

\iffalse
\begin{scriptsize}
\begin{verbatim}
- We delve deep into the mitigation mechanisms, and we focus on two things:
1. what secret can be leaked to bypass the protection mechanism
2. how to leak the secret via speculative execution attacks
- we summarize our analysis result in table 2
- we find there exist two attack strategies, we identify their working conditions, and applicable to which mitigation mechanisms
1. attack strategy 1: use the basic spectre v1 attack and its variations
explain the satisfiable condition
secret stored or encoded in virtual memory, this include stack canary, and aslr
2. attack strategy 2: speculative crash
if secret is not stored in virtual memory, either metadata data or randomization, 
using incorrect metadata or offset, will cause check failure, 
if the failed check can cause speculative execption, which is only handled at the head of RoB -> we can leak the check results via ....
Table 2 summarizes for each potentially vulnerable mechanism, we list 
the secret data, whether the data is stored in memory, whether failed security check can generate speculative exception,
we also list which attack strategy can work on ...
We provide a detailed discusson on them in 4 groups as below based on which attack strategies work twoards them.

\end{verbatim}
\end{scriptsize}
\fi


\iffalse
\begin{table}[t]
    \centering
    \caption{}
    \mengjia{1. secret stored in memory -> secret stored/encoded in memory, in this way, we should also check ASLR, Morpheus, or maybe something more. These stuff can be leaked via secondary software vulnerabilities;\\
    2. ASLR can be leak via both transient de-refernece and crash, same thing applies to morphedus. Note that Speculative Probing have multiple probe methods.}
    \small
    \begin{tabular}{|c|c||c|c||c|c|}\hline
    & &  \multicolumn{2}{c||}{What to Leak}  & \multicolumn{2}{c|}{How to Leak}  \\\cline{3-6}
    &Scheme &  secret  & in virtual & Transient  & Transient  \\ 
    &       &   &  memory? & De-reference & Crash \\ \hline\hline
    1 & Stack  & Canary & \checkmark &  \checkmark & x  \\
     & Canary~\cite{stackguard_canaries} &   &   &   &  \\\hline
    %Protection & & & & \\\hline
    2 & ASLR & Segment  & \checkmark & \checkmark & \checkmark \\\
    & \cite{aslr?} & Offset & & & \\\hline
    3 & Morpheus & Segment   & \checkmark & \checkmark & \checkmark \\\
    & \cite{morpheus}& Offset & & & \\\hline
    4 & AOS~\cite{aos} & PAC & \checkmark & \checkmark & x\\\hline
    5 & Califorms & Security & x & \checkmark & x \\\
    & \cite{califorms}& bits~\footnote{califorms-sentinel in L2 and beyond, and califorms-bitvecotr in L1} & & & \\\hline
    6 & ARM  & PAC & x & x & \checkmark\\
    &PA~\cite{armpa} &  &  &  & \\\hline
    7 & C3~\cite{c3} & Cryptogra-  & x & x & \checkmark\\
    & & phic Address & & & \\\hline
    8 & ARM  & Memory   & x & x & \checkmark \\
     & MTE~\cite{armmte} &  Tag  &  &  &  \\\hline
    9 & SPARC  & Memory  & x & x & \checkmark \\
     & ADI~\cite{adi} &  Tag &  &  &  \\\hline
    10 & No-FAT & Allocation   & x & x & \checkmark \\
    &\cite{no-fat} &  Tag  &  &  &  \\\hline
    \end{tabular}
    \label{tab:comparison}
\end{table}
\fi
